On The Reliability Function of Discrete Memoryless Multiple-Access Channel with Feedback

The reliability function of a channel is the maximum achievable exponential rate of decay of the error probability as a function of the transmission rate. In this work, we derive bounds on the reliability function of discrete memoryless multiple-access channels (MAC) with noiseless feedback. We show that our bounds are tight for a variety of MACs, such as $m$-ary additive and two independent point-to-point channels. The bounds are expressed in terms of a new information measure called ``variable-length directed information". The upper bound is proved by analyzing stochastic processes defined based on the entropy of the message, given the past channel's outputs. Our method relies on tools from the theory of martingales, variable-length information measures, and a new technique called time pruning. We further propose a variable-length achievable scheme consisting of three phases: (i) data transmission, (ii) hybrid data-confirmation, and (iii) full confirmation. We show that two-phase-type schemes are strictly suboptimal in achieving the MAC's reliability function. Moreover, we study the shape of the lower-bound and show that it increases linearly with respect to a specific Euclidean distance measure defined between the transmission rate pair and the capacity boundary. As side results, we derive an upper bound on the capacity of MAC with noiseless feedback and study a new problem involving a hybrid of hypothesis testing and data transmission.

==> SupportingHP_-_Copy.tex <==
\section{Characterization of the Feedback Capacity Region Via Supporting Hyper-Plans} \label{app:CFB supporting HYP}

%\%paragraph{Standard multi-letter characterization of the feedback capacity:}

%For any positive integer $L$, let $\mathcal{P}_L$ be the set of all $P_{X_1^LX_2^LY^L}$ that factors as 
%\begin{align}\label{eq: factorization of P}
%\prod_{l=1}^L P_{1,l}(x_{1l}| x_1^{l-1} y^{l-1})P_{2,l}(x_{2l}| x_2^{l-1} y^{l-1})P_{Y|X_1X_2}(y_l|x_{1, l}x_{2,l}),
%\end{align}
%where $P_{Y|X_1X_2}$ is the conditional distribution of the MAC channel. 
For any $L\in \NN$ and  $P\in \mathcal{P}_{L}$, define 
\begin{align*}
\mathcal{C}_L(P)\deq \bigg\{(R_1, R_2)\in [0,\infty)^2: R_1 &\leq I_L(X_1 \rightarrow Y|| X_2),\\
 R_2 &\leq I_L(X_2 \rightarrow Y|| X_1),\\\numberthis \label{eq:Cp}
  R_1+R_2 &\leq I_L(X_1 X_2 \rightarrow Y)\quad \bigg\},
\end{align*}
where $I_L$ is the normalized $L$-letter directed (casually conditioned) mutual information defined as
\begin{align}\label{eq: normalized direct info}
I_L(X\rightarrow Y|| Z)=\frac{1}{L}I(\mathbf{X}^L \rightarrow \mathbf{Y}^L \| \mathbf{Z}^L).
\end{align}

It is known that \cite{Kramer-thesis} the feedback-capacity region of a two-user discrete memoryless MAC with feedback and via fixed-length codes is given by
\begin{align*}
\mathcal{C}_{FB}=ccl\bigg[\bigcup_{L\in \NN}\bigcup_{P\in \mathcal{P}_L}\mathcal{C}(P)\bigg].
\end{align*}
 
In what follows we provide an alternative characterization used for our achievability scheme. 

\noindent{\bf Alternative characterization with time-sharing variable:}

Let $\mathcal{Q}$ be a finite set. It suffices to assume $|\mathcal{Q}|= 3$. For any positive integer $L$, define  $\mathcal{PQ}_L$ as the set of 
all joint distributions $P_{QX_1^LX_2^LY^L}$ such that the conditioned distribution $P_{X_1^LX_2^LY^L|Q=q}\in \mathcal{P}_L$ for any $q\in \mathcal{Q}$.

Define the general conditional directed mutual information as 
\begin{align}\label{eq: conditional direct info}
I(\mathbf{X}^L \rightarrow \mathbf{Y}^L|| \mathbf{Z}^L| Q)= \sum_{\ell=1}^L I(\bfX^\ell; Y_\ell| \bfY^{\ell-1} \bfZ^\ell Q).
\end{align}
Here $Z^L$ is conditioned casually, whereas $Q$ is conditioned non-casually.  
Now, define 

\begin{align*}
\mathcal{C}'_{FB}=cl\bigg[\bigcup_{L\in \NN}\bigcup_{P\in \mathcal{PQ}_L}\bigg\{(R_1, R_2)\in [0,\infty)^2: R_1 &\leq I_L(X_1 \rightarrow Y|| X_2~|Q),\\
 R_2 &\leq I_L(X_2 \rightarrow Y|| X_1~|Q),\\\numberthis \label{eq:C_FB prime}
  R_1+R_2 &\leq I_L(X_1 X_2 \rightarrow Y|Q)\quad \bigg\}\bigg],
\end{align*}
where \textit{cl} means closure.
\begin{lem}\label{lem:C_FB prime}
$\mathcal{C}'_{FB}=\mathcal{C}_{FB}$.
\end{lem}
\begin{proof}
First, we prove that $\mathcal{C}'_{FB}$ is achievable.  Let $(R_1, R_2)$ be a rate-pair inside $\mathcal{C}'_{FB}$. Then, there exists $L>0$ and $P\in \mathcal{PQ}_L$ such that the inequalities in \eqref{eq:C_FB prime} are satisfied. Note that, 
\begin{align*}
I_L(X_1 \rightarrow Y|| X_2~|Q) &= \sum_{q\in \mathcal{Q}} P_Q(q) I_L(X_1 \rightarrow Y|| X_2~|Q=q)\\
&=\sum_{q\in \mathcal{Q}} I_L(X_1 \rightarrow Y|| X_2)_{P_{X_1^LX_2^LY^L|Q=q}}.
\end{align*}
Similarly, other mutual information quantities are decomposed. By assumption, $P_{X_1^LX_2^LY^L|Q=q}\in \mathcal{P}_L$. Hence, $C(P_{X_1^LX_2^LY^L|Q=q})$ as in \eqref{eq:Cp} is a well-defined set. Now, let $(R_{1,q}, R_{2,q})$ be a rate-pair inside this set such that 
\begin{align*}
(R_1, R_2)=\sum_{q\in \mathcal{Q}}P_Q(q) (R_{1,q}, R_{2,q}).
\end{align*}
Since $(R_{1,q}, R_{2,q})$ are achievable, their convex combination is also achievable. Hence, $(R_1,R_2)\in \mathcal{C}_{FB}$; implying that $\mathcal{C}'_{FB}\subseteq \mathcal{C}_{FB}$.

Next, we prove that $\mathcal{C}_{FB}\subseteq \mathcal{C}'_{FB}$. Let $(R_1, R_2)\in \mathcal{C}_{FB}$. Then, by Caratheodory's theorem, $(R_1,R_2)$ can be written as a convex combination of at most three rate-pairs in $\bigcup_{L\in \NN}\bigcup_{P\in \mathcal{P}_L}\mathcal{C}(P)$. Denote such rate pairs by $(R_{1,q}, R_{2,q})$. Hence, there exist a distribution $P_Q$ so that
\begin{align*}
(R_1,R_2)=\sum_{q}P_Q(q)(R_{1,q}, R_{2,q}).
 \end{align*}
In addition, for each $q$, there exists $L_q>0$ and a $L_q$-letter distribution $P_{q, L_q}$ so that $(R_{1,q}, R_{2,q})\in \mathcal{C}(P_{q, L_q})$. Let $L=\prod_q L_q$. Then, there exists a conditional $L$-letter distribution $P_{X_1^LX_2^LY^L|Q}$ such that 
\begin{align*}
 P_{X_1^LX_2^LY^L|Q=q}=\prod_{m=1}^{L/L_q} P_{q, L_q}, \quad \text{for all} ~q\in \mathcal{Q}
 \end{align*}
By construction, $ P_{X_1^LX_2^LY^L|Q=q}\in\mathcal{P}_L$ and $(R_{1,q}, R_{2,q})\in \mathcal{C}(P_{X_1^LX_2^LY^L|Q=q})$. Therefore, we obtain that 
\begin{align*}
R_{1} &\leq \sum_{q} P_Q(q) I_L(X_1 \rightarrow Y|| X_2~|Q=q)=I_L(X_1 \rightarrow Y|| X_2~|Q),\\
R_{2} &\leq \sum_{q} P_Q(q) I_L(X_2 \rightarrow Y|| X_1~|Q=q)=I_L(X_2 \rightarrow Y|| X_1~|Q),\\
R_1+R_2 &\leq \sum_{q} P_Q(q) I_L(X_1 X_2 \rightarrow Y|Q=q)=  I_L(X_1 X_2 \rightarrow Y|Q).
\end{align*}
As a result, $(R_1, R_2)\in \mathcal{C}'_{FB}$; implying that $\mathcal{C}_{FB}\subseteq \mathcal{C}'_{FB}$. 
\end{proof}


\noindent{\bf Characterization of the capacity via supporting hyperplanes:}
Now we are ready to prove Theorem \ref{thm:capacity C lambda}.
For any $P\in \mathcal{PQ}_L$, define
\begin{align*}
E(P)\deq \bigg\{(R_1, R_2, R_3)\in [0,\infty)^3: R_1 &\leq I_L(X_1 \rightarrow Y|| X_2~| Q),\\
 R_2 &\leq I_L(X_2 \rightarrow Y|| X_1~| Q),\\
  R_3 &\leq I_L(X_1 X_2 \rightarrow Y | Q)\quad \bigg\}.
\end{align*}
and let 
\begin{align*}
E=cl\bigg[\bigcup_{L\in \NN}\bigcup_{P\in \mathcal{PQ}_L}E(P)\bigg].
\end{align*}
\begin{lem}
$E$ is a convex set in $\RR^3$.
\end{lem}
\begin{proof}
The proof follows from the convexifying random variable $Q$  in  the mutual information quantities and from Caratheodory's theorem ( implying that it is sufficient to have $|\mathcal{Q}|=3$).
\end{proof}

Let $\underline{\lambda} \in \Delta^3$, where $\Delta^3$ is the simplex of vectors $v\in [0,1]^3$ satisfying $\sum_iv_i=1$. Define, 
\begin{align*}
C_{\underline{\lambda}} \deq \sup_{L\in \NN}\sup_{P\in \mathcal{PQ}_L} \Big(\lambda_1 I_L(X_1 \rightarrow Y|| X_2~| Q)+\lambda_2 I_L(X_2 \rightarrow Y|| X_1~| Q)+\lambda_3 I_L(X_1 X_2 \rightarrow Y | Q)\Big)
\end{align*}
With that let
\begin{align*}
E' \deq \bigg\{(R_1, R_2, R_3)\in [0,\infty)^3: \forall \underline{\lambda} \in \Delta^3, \sum_{i}\lambda_i R_i \leq C_{\underline{\lambda}}\bigg\}
\end{align*}

\begin{lem}[Salehi'78]
$E'=E$
\end{lem}

Next, define 
\begin{align*}
\mathcal{D}\deq \Big\{(R_1, R_2)\in [0,\infty)^2: (R_1, R_2, R_1+R_2)\in E\Big\}. 
\end{align*}

\begin{lem}
$\mathcal{D}=\mathcal{C}_{FB}$
\end{lem}
\begin{proof}
Due to its definition, $\mathcal{C}'_{FB}=\mathcal{D}$. Hence, this lemma follows from  Lemma \ref{lem:C_FB prime}, indicating that $\mathcal{C}_{FB}=\mathcal{C}'_{FB}=\mathcal{D}$. 
\end{proof}

Consequently, the lemmas above imply another characterization of the capacity region via supporting hyperplanes. That is the set of rate pairs $(R_1, R_2)$ such that for all $\underline{\lambda}\in \Delta^3$ the following inequality holds
\begin{align*}
\lambda_1 R_1 + \lambda_2 R_2+\lambda_3(R_1+R_2) \leq \mathcal{C}_{\underline{\lambda}}.
\end{align*}
With that the proof of Theorem \ref{thm:capacity C lambda} is complete.


==> ThreePhaseUP.tex <==
\subsection{Upper Bounds}\label{subsec:threephase up}
Before proceeding with the results we establish some additional notation. %Consider a pair of random sequences $(X^n,Y^n)\sim P_{X^nY^n}$. Let $X_r^*$ be the MAP estimation of $X_r$ from observation $Y^{r-1}$, that is $X_r^* =\argmax_{x} \prob{X_r = x | Y^{r-1}}$. %\red{[AA: The $\prob$ environment is a bit weird...better $\mathbb{P}()$. Also shouldn't the conditioning be just $Y^{r-1}$? ]}.
% Then, define 
%\begin{align*}
%P^*_{Y_r|Y^{r-1}}(y_r| y^{r-1}) \deq P_{Y_r| X_r, Y^{r-1}}(y_r |x^*_r, y^{r-1}), 
%\end{align*}
%for all values of $y^{r-1}$,and  $y_r$. Intuitively, $P^*_{Y_r|Y^{r-1}}$ is the distribution of $Y_r$ conditioned on $Y^{r-1}$ and the event that MAP correctly finds $X_r$. Alternatively, when MAP' estimation is wrong, then we define   the following distribution
%\begin{align*}
%\tilde{P}_{Y_r|Y^{r-1}}(y_r| y^{r-1}) \deq P_{Y_r| X_r, Y^{r-1}}(y_r | X_r \neq x^*_r, Y^{r-1}= y^{r-1}).
%\end{align*}
%With this notation, we define the directed KL-divergence as 
For  any $P \in \PMAC$, let $\Qbar{1}_r\deq P_{Y_r|X_{1, r},Y^{r-1}}$ and $\Qbar{2}_r\deq P_{Y_r|X_{2, r},Y^{r-1}}$ be the effective channel from the first user's perspective at time $t=r$. Then, for  any $y^{r-1}\in \mathcal{Y}^{r-1}$, define
\begin{align*}
    \D_r^1(y^{r-1})  \deq \max_{x_1, x'_1}\sup_{P_{X'_2|Y^{r-1}}} D_{KL}\Big( \Qbar{1}_r(\cdot | x_1, y^{r-1})~\|~ \Qbarp{1}_r(\cdot | x'_1, y^{r-1}) \Big),
\end{align*}
where $\Qbarp{1}_r$ is an effective channel of the first user  with the distribution of the second user chosen as $P_{X'_2|Y^{r-1}}$. Similarly, let $\Qbar{2}_r\deq P_{Y_r|X_{2, r},Y^{r-1}}$ be the effective channel from the second user's perspective at time $t=r$, and define 
\begin{align*}
    \D_r^2(y^{r-1}) \deq \max_{x_2, x'_2}\sup_{P_{X'_1|Y^{r-1}}} D_{KL}\Big( \Qbar{2}_r(\cdot | x_2, y^{r-1})~\|~ \Qbarp{2}_r(\cdot | x'_2, y^{r-1}) \Big).
\end{align*}
Moreover, define 
\begin{align*}
    \D^3 \deq \max_{x_1, x'_1}\max_{x_2, x'_2} D_{KL}\Big( Q(\cdot | x_1, x_2)~\|~ Q(\cdot | x'_1, x'_2) \Big).
\end{align*}
% Lastly, define 
% \begin{align*}
% %\D_r^i \deq \max_{x_i\in \mathcal{X}_i} D_{KL}\Bigg(P_{Y_r|X_{i,r}, Y^{r-1}}(\cdot | x^*_{i,r}, y^{r-1})~~ \Big\|~~ P_{Y_r|X_{i,r}k, Y^{r-1}}(\cdot | x_i, y^{r-1})\Bigg),
% D_i(X^{n} \rightarrow Y^n)  \deq \max_{x^n,z^n}\sum_{r=1}^n  D_{KL}\qty(P_{Y_r|X_{r},Y^{r-1}}(\cdot |x_r, Y^{r-1})~~ \Big\|~~ P_{Y_r|X_{r},Y^{r-1}}(\cdot |z_r, Y^{r-1}) ~\Big|~ Y^{r-1}).  
% \end{align*}
% Intuitively, $D(X^{n} \rightarrow Y^n) $ measures the sum of the expected ``distance" between the channel's probability distribution conditioned on the MAP symbol versus the worst symbol, across different times $r\in [1:n]$. Now, given an third random variable $Z$, and a joint distribution $P_{X^n,Y^n,Z}$, we can define the conditional version of  the directed KL-divergence as 
% \begin{align*}
% D(X^{n} \rightarrow Y^n | Z)  \deq \max_{x^n} \sum_{r=1}^n  D_{KL}\Bigg(P_{Y_r|X_{r},Y^{r-1},Z}(\cdot |X_r^*, Y^{r-1}, Z)~~ \Big\|~~ P_{Y_r|X_{r},Y^{r-1},Z}(\cdot |x_r, Y^{r-1}, Z) ~\Big|~ Y^{r-1}, Z\Bigg).  
% \end{align*}
With this notation, we are ready to present the main result of this section. 

\begin{theorem}\label{thm:upper bound three phase}
The reliability function of a MAC channel is bounded from above as 
\begin{align*}
E(R_1,R_2) \leq 
E^{ub}(R_1,R_2) :=
\sup_{P \in \PMAC} \sup_{\substack{ T:\\  T\leq N_P}} \sup_{\substack{ T_1,T_2, T_3 :\\ T_i\leq T} }  \min_{i\in \{1,2,3\}} \left\{D^i(P) \Big(1 - \frac{R_i}{I^i(P)}\Big)\right\},
\end{align*}
where $R_3=R_1+R_2$, and $I^i(P)$ and $D^i(P)$ are defined as
\begin{align*}
I^1(P) &= \frac{1}{\EE[T_1]}    I(X_1^{T_1} \rightarrow Y^{T_1}|| X_2^{T_1}), \qquad    &     D^1(P) &=\frac{1}{\EE[T-T_1]} \EE\Big[ \sum_{r=T_1}^T   \D_r^1(Y^{r-1})   \Big] \\%D(X_{1, T_1}^{T} \rightarrow Y_{T_1}^{T})   \\
I^2(P) &= \frac{1}{\EE[T_2]}    I(X_2^{T_2} \rightarrow Y^{T_2}|| X_1^{T_2} ), \qquad    &     D^2(P) &=\frac{1}{\EE[T-T_2]} \EE\Big[ \sum_{r=T_2}^T   \D_r^2(Y^{r-1})   \Big] \\%D(X_{2, T_2}^{T} \rightarrow Y_{T_2}^{T}  )   \\
I^3(P) &= \frac{1}{\EE[T_3]}    I(X_1^{T_3}X_2^{T_3} \rightarrow Y^{T_3}),    \qquad    &     D^3(P) &=D^3. \\ %\frac{1}{\EE[T-T_3]}\EE\Big[ \sum_{r=T_3}^T   \D_r^3   \Big] \\% D(X_{1, T_3}^{T}X_{2, T_3}^{T} \rightarrow Y_{T_3}^{T} )   
\end{align*}
\end{theorem}

%\red{Making a corollary to re-derive the two-phase outer bound.}
%\red{A paragraph discussing the overall strategy of the proofs. Say about the three phase scheme, and strategy.}
%The rest of this section focuses on the steps for proving this result.


==> figures/MATH_template.tex <==
\usepackage{tikz}
%\usepackage{mathdots}
\usepackage[utf8]{inputenc}
%\usepackage[ margin=1in ]{geometry}

\usepackage{amsmath} \usepackage{amsthm} \usepackage{amsfonts} \usepackage{amssymb} 
\usepackage{epstopdf}
%\usepackage{mathtools}
\usepackage{graphicx}
%\usepackage{relsize}
%\usepackage{xy}
%\input{xypic}
\usepackage{bbm}
%\setlength{\footskip}{20pt}

\usepackage{enumerate}

%\onecolumn

%\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{definition}{Definition}

\theoremstyle{definition}
\newtheorem{example}{Example}
\newtheorem{conjecture}{Conjecture}
\newtheorem{question}{Question}
\newtheorem{problem}{Problem}
\newtheorem*{prob*}{Problem}
\newtheorem{fact}{Fact}


\theoremstyle{remark}
\newtheorem{remark}{Remark}
\newtheorem{rems}{Remarks}
\newtheorem{para}{}
\newtheorem{summary}{Summary}



\renewcommand{\Re}[1]{\ensuremath{\operatorname{Re}\left\{#1\right\}}}
\renewcommand{\Im}[1]{\ensuremath{\operatorname{Im}\left\{#1\right\}}}

\newcommand{\BigO}[1]{\ensuremath{\operatorname{O}\bigl(#1\bigr)}}

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}



\global\long\def\Z{\mathrm{{\bf Z}}}
\global\long\def\N{\mathrm{{\bf N}}}
\global\long\def\Gal{\mathrm{Gal}}
\global\long\def\RR{\mathbb{R}}
\global\long\def\CC{\mathbb{C}}
\global\long\def\NN{\mathbb{N}}
\global\long\def\QQ{\mathbb{Q}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\EE{\mathbb{E}}
\global\long\def\PP{\mathbb{P}}
\global\long\def\FF{\mathbb{F}}

 \global\long\def\dd{\cdots}
\global\long\def\normal{\triangleleft}

\newcommand*{\Scale}[2][4]{\scalebox{#1}{\ensuremath{#2}}}%

==> figures/new_journal_template.tex <==
%=============================================================================
%------------------  Basic Packages -----------------------------------------
%=============================================================================

\usepackage{amsmath}
\usepackage{amsfonts}

\usepackage{mathrsfs}
\usepackage{tikz}
%\usepackage{mathdots}
\usepackage[utf8]{inputenc}
%\usepackage[ margin=1in ]{geometry}
\usepackage{amsfonts} 
\usepackage{epstopdf}
\usepackage{mathtools}
\usepackage{graphicx}
%\usepackage{relsize}
%\usepackage{xy}
%\input{xypic}
\usepackage{bbm}
%\setlength{\footskip}{20pt}
\usepackage{enumerate}
\usepackage{epsf,verbatim,amssymb,array,cite,multicol,multirow}  
\usepackage{psfrag,bm,xspace}
%\usepackage{slashbox}
\usepackage{hhline}
\usepackage{mathabx}
\usepackage{xstring}
\usepackage{ifthen}

\pagestyle{plain}
\usepackage{amsthm}

%\def\old@comma{,}
%\catcode`\,=13
%\def,{%
%  \ifmmode%
%    \old@comma\discretionary{}{}{}%
%  \else%
%    \old@comma%
%  \fi%
%}
%\makeatother

%=============================================================================
%---------------------------  Quantum Packages  ------------------------------
%=============================================================================
%\usepackage{physics}


%=============================================================================
%------------------  Basic Theorem Enviroments -----------------------------------------
%=============================================================================

%\newtheorem{thm}{Theorem}
\newtheorem{theorem}{Theorem}
%
\newtheorem{lem}{Lemma}
%%\newtheorem{lemma}{Lemma}
%
\newtheorem{corollary}{Corollary}
%\newtheorem{cor}{Corollary}
%
\newtheorem{fact}{Fact}
\newtheorem{proposition}{Proposition}
%\newtheorem{claim}{Claim}
%
%
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
%\newtheorem{conjecture}{Conjecture}
%\newtheorem{question}{Question}
%\newtheorem{problem}{Problem}
%\newtheorem*{prob*}{Problem}
%\newtheorem{algorithm}{Algorithm}
%
\theoremstyle{remark}
\newtheorem{remark}{Remark}
%\newtheorem{rem}{Remark}


\newtheorem{innercustomlem}{Lemma}
\newenvironment{customlem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomlem}

%-----------------------------------------------------------------------------------------

% makes automatic splits of equations and commas
%%\allowdisplaybreaks 
\makeatletter
\def\old@comma{,}
\catcode`\,=13
\def,{%
  \ifmmode%
    \old@comma\discretionary{}{}{}%
  \else%
    \old@comma%
  \fi%
}
\makeatother

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

%=============================================================================
%------------------  Tracking the changes  -----------------------------------
%=============================================================================
\usepackage{xcolor}
\definecolor{darkblue}{rgb}{0.1,0.1,0.8}
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\definecolor{britishracinggreen}{rgb}{0.0, 0.26, 0.15}
\definecolor{calpolypomonagreen}{rgb}{0.12, 0.3, 0.17}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
	\definecolor{cadmiumgreen}{rgb}{0.0, 0.42, 0.24}
\definecolor{burgundy}{rgb}{0.5, 0.0, 0.13}
\usepackage{etoolbox}

\providetoggle{Blue_revision}
\settoggle{Blue_revision}{true}
\newcommand{\revcol}{\iftoggle{Blue_revision}{\color{blue}}{ }}
\newcommand{\add}[1]{\iftoggle{Blue_revision}{{\color{darkblue}#1}}{ }}
\newcommand{\change}[2]{\iftoggle{Blue_revision}{{\footnotesize \color{brickred}#1}{\color{darkblue}#2}}{ }}

%================  Tracking Multiple Versions ==================================
\providetoggle{Track}
\settoggle{Track}{true}
\newcommand{\addv}[3]{%
	\iftoggle{Track}{%
    	\IfEqCase{#1}{%
       	 	{a}{\ifthenelse{\equal{#2}{ON}}{{\color{cadmiumgreen}#3}}{#3}}%
        	{b}{\ifthenelse{\equal{#2}{ON}}{{\color{brickred}#3}}{#3}}%
       		{c}{\ifthenelse{\equal{#2}{ON}}{{\color{burgundy}#3}}{#3}}%
        	% you can add more cases here as desired
    	}[\PackageError{tree}{Undefined option to tree: #1}{}]%
	}{#3}%
}

%\newcommand{\add}[3]{\iftoggle{#1}{{\color{#2}#3}}{ }}
%\newcommand{\change}[4]{\iftoggle{#1}{{\footnotesize \color{#2}#3}{\color{darkblue}#4}}{ }}



%================  Hyper Cross Refrrences ==================================

 \usepackage{hyperref}
\usepackage{xcolor}
\definecolor{DarkGreen}{rgb}{0,0.6,0}

\hypersetup{
colorlinks=true, %
  pdfstartview={FitH},
    linkcolor=red,
    citecolor=blue,
    urlcolor={blue!80!black}
}


\usepackage{graphicx}

%=============================================================================
%---------  Labeling equality and inequalities  ------------------------------
%=============================================================================


\newcounter{relctr} %% <- counter for relations
\everydisplay\expandafter{\the\everydisplay\setcounter{relctr}{0}} %% <- reset every eq
\renewcommand*\therelctr{\alph{relctr}} %% <- label format

\newcommand\mystackrel[2]{%
  \begingroup
    \refstepcounter{relctr}%
    \stackrel{\text{(\alph{relctr})}}{\mathstrut{#1}}%
    \originallabel{#2}%
  \endgroup
}
\AtBeginDocument{\let\originallabel\label} %% <- store original definition



==> proofs/Proof_lem_log_old.tex <==
\section{Proof of Lemma \ref{lem: log drift MAC FB} }\label{appx: proof of lem log drift}
\begin{IEEEproof}
We start with the case $i=1$. The proof for the other two cases follows from the same argument.  Define the following quantities
\begin{align*}
%f_{i|m}&=P(W_1=i| Y^t=y^t, W_2=m)\\
\mu_{1}(w)&=\prob{W_1=w| Y^{r-1}=y^{r-1}}\\
\mu_{1}(w, y_{r})&=\prob{W_1=w| Y^{r-1}=y^{r-1},Y_{r}=y_{r}}\\
Q^1_{w}(y_{r})&=\prob{Y_{r}=y_{r}|W_1=w, Y^{r-1}=y^{r-1}},
\end{align*}
where $w\in [1:M_1], y_{t+1}\in \mathcal{Y}$. 
 
Let $\Wstar \in [1: M_1]$ be the most likely message condition on $y^{r-1}$. That is $\wstar = \argmax_{w\in [1: M_1]}\mu_{1}(w)$.
First, we show that having $\Htld^1_{r-1} < \epsilon, \epsilon\in [0,1)$ implies that $\mu_1(\wstar)= 1-\eta_1(\epsilon)$ with $\eta_1$ being a function satisfying $\lim_{\epsilon \rightarrow 0} \eta_1(\epsilon) =0.$ The argument is as follows:
 
Using the grouping axiom we have
\begin{align}\label{eq:Htld eq 1}
\Htld^1_{r-1}=H(W_1|y^{r-1})=h_b( \mu_1(w^*_{1,r}))+(1-\mu_1(w^*_{1,r}))H(\hat{W}_1), 
%\geq h_b( \mu_1(w^*_{1,r}))+(1-\mu_1(w^*_{1,r}))
\end{align}
where $\hat{W}_1$ is a random variable with probability distribution $P(\hat{W}_1=w)=\frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})}, ~w\in [1:M_1], w\neq w^*_{1,r}$. Hence, having $\Htld^1_{r-1}\leq \epsilon$ implies that $h_b(\mu_1(\wstar))\leq \epsilon$.
Taking the inverse image of $h_b$ implies that either $\mu_1(\wstar)\geq 1-h_b^{-1}(\epsilon)$ or $\mu_1(\wstar)\leq h_b^{-1}(\epsilon)$, where $h_b^{-1}:[0,1]\rightarrow [0,\frac{1}{2}]$ is the lower-half inverse function of $h_b$.  We show that the second  case is not feasible. For this purpose, we show that the inequality $\mu_1(\wstar)\leq h_b^{-1}(\epsilon)$ implies that $\Htld^1_{r-1}\geq 1$ which is a contradiction  with the original assumption $\Htld^1_{r-1} \leq \epsilon < 1$. This statement is proved in the following proposition. With this argument, we conclude that $\Htld^1_{r-1}\leq \epsilon$ implies that $\mu_1(\wstar)\geq 1-\eta_1(\epsilon)$, where $\eta_1(\cdot) = h_b^{-1}(\cdot)$.

\begin{proposition}
Let $W$ be a random variable taking values from a finite set $\mathcal{W}$. Suppose that $P_W(w)\leq \frac{1}{2}$ for all $w\in \mathcal{W}$. Then $H(W)\geq 1$. 
\end{proposition}
\begin{proof}
The proof follows from an induction on $|\mathcal{W}|$. For $|\mathcal{W}|=2$ the condition in the statement implies that $W$ has uniform distribution and hence $H(W)=1$ trivially. Suppose the statement holds for $|\mathcal{W}|=n-1$. Then, for $|\mathcal{W}|=n$.  Sort elements of $\mathcal{W}$ in an descending order according to $P_W(w)$, from the most likely (denoted by $w_1$) to the least likely ($w_n$). If $P_W(w_n)=0$, then the statement holds trivially from the induction's hypothesis.  Suppose $P_W(w_n)>0$. In this case,  by the grouping axiom, we can reduce  $H(W)$ by increasing $P_W(w_1)$ and decreasing $P_W(w_n)$ so that $P_W(w_1)+P_W(w_n)$ remains constant. In that case, either $P_W(w_n)$ becomes zero or $P_W(w_1)$ reaches the limit $\frac{1}{2}$. The first case happens if $P_W(w_1)+P_W(w_n)\leq \frac{1}{2}$. For that, the statement $H(W)\geq 1$ follows from the induction's hypothesis, as there are only $(n-1)$ elements with non-zero probability.  It remains to consider the second case in which $P_W(w_1)=\frac{1}{2}$ and $P_W(w_n)>0$. Again, we can further reduce the entropy by increasing $P_W(w_2)$ and decreasing $P_W(w_n)$ while $P_W(w_2)+P_W(w_n)$ remains constant. Observe that $P_W(w_2)+P_W(w_n)\leq \frac{1}{2}$ as $\sum_{i=2}^n P_W(w_i) = 1-P_W(w_1)=\frac{1}{2}$ and $p_W(w_i)>0$.  Hence, after this redistribution process $P_W(w_n)$ becomes zero. Then, the statement $H(W)\geq 1$ follows from the induction's hypothesis, as there are only $(n-1)$ elements with non-zero probability.
\end{proof}

%By grouping the messages $w\neq \wstar$ into a one combo message, we can write 
%\begin{align*}
% \epsilon \geq \Htld^1_{r-1}\geq h_b(\mu_1(\wstar)).
% \end{align*} 
% Taking the inverse image of $h_b$ implies that $\mu_1(\wstar)\geq 1-h_b^{-1}(\epsilon)$ or $\mu_1(\wstar)\leq h_b^{-1}(\epsilon)$. The second inequality is not feasible because otherwise if $\epsilon=0$ then $\mu_1(\wstar)=0$ which is a contradiction as $\wstar$ is the MAP message. Hence, $\mu_1(\wstar)\geq 1-h_b^{-1}(\epsilon)$. Therefore, there exists a function $o_1(\epsilon)$ such that $\mu_1(\wstar)=1-o_1(\epsilon)$ and $0\leq o_1(\epsilon)\leq h_b^{-1}(\epsilon)$.

Next, we analyze the log-drift. Fix $\delta\in (0,1/2)$, and let $\mathcal{Y}_\delta :=\{y_r\in \mathcal{Y}: P(y_r|y^{r-1})>\delta\}.$ Then,

\begin{align*}
\EE[\log \Htld^1_{r-1}-\log \Htld^1_{r}|\mathcal{F}_{r-1}] &\leq \sum_{y_r\in \mathcal{Y}_\delta} P(y_r|y^{r-1}) \log \frac{\Htld^1_{r-1}}{\Htld^1_{r}(y_r)}+\delta  \sum_{y_r\notin \mathcal{Y}_\delta} \Big|\log \frac{\Htld^1_{r-1}}{\Htld^1_{r}(y_r)}\Big| \\
&\leq \sum_{y_r\in \mathcal{Y}_\delta} P(y_r|y^{r-1})\log \frac{\Htld^1_{r-1}}{\Htld^1_{r}(y_r)}+\delta  \eta |\mathcal{Y}|,
\end{align*}
where $\eta$ is given in Lemma \ref{rem: H_t+1 - H_tis bounded}.
%there exist sufficiently small $\epsilon'\in (0,1)$ (as a function of $\epsilon$) such that $\mu_1(w^*_{1,r})= 1-\epsilon'$ and $\mu_1(w)\leq \frac{\epsilon'}{M_1-1}$ for all $w\neq w^*_{1,r}$. 
We proceed  by applying Lemma 7 in \cite{Burnashev} stated below.
 %\begin{customlem}{7}[\cite{Burnashev}]
For any non-negative sequence of numbers $p_\ell,\mu_i$ and $\beta_{i,l}, \ell \in [1:L], i\in [1:N]$ the following inequality holds
\begin{align*}
\sum_{\ell=1}^L p_\ell \log\Big( \frac{\sum_{i=1}^N \mu_i}{\sum_{i=1}^N \beta_{i,\ell}}  \Big) \leq \max_{i} \sum_{\ell=1}^L p_{\ell} \log \frac{\mu_i}{\beta_{i,\ell}}.
\end{align*}
%\end{customlem}

 By the definitions of $\Htld^1_{r-1}$ and  $\Htld^1_{r}$, we have that 
\begin{align*}
\EE[\log \Htld^1_{r-1}-\log \Htld^1_{r}|\mathcal{F}_{r-1}] &\leq \sum_{y_r\in \mathcal{Y}_\delta} P(y_r|y^{r-1}) \log\Big(\frac{-\sum_{w} \mu_1(w)\log \mu_1(w) }{-\sum_{w}\mu_1(w,y_r)\log \mu_1(w,y_r)}\Big) +\delta \eta |\mathcal{Y}|\\\numberthis\label{eq:log drift gamma}
& \leq  \max_{w} \Gamma(w) +\delta \eta |\mathcal{Y}|,
\end{align*}
where 
\begin{align*}
\Gamma(w) = \sum_{y_r\in \mathcal{Y}_\delta} P(y_r|y^{r-1}) \log \frac{-\mu_1(w)\log \mu_1(w)}{-\mu_1(w,y_r)\log \mu_1(w,y_r)}.
\end{align*}



Note that 
\begin{align}\label{eq:mu wstar and y}
\mu_{1}(w, y_{r})&=\frac{\mu_1(w) Q_w(y_r)}{P(y_r|y^{r-1})}.
\end{align}
Therefore, for a fixed $w\neq \wstar$ we have that
\begin{align}\nonumber
-\Gamma(w) &= \sum_{y_r\in \mathcal{Y}_\delta} P(y_r|y^{r-1}) \log\bigg[ \frac{Q_w(y_r)}{ P(y_r|y^{r-1})}\Big(1+\frac{\log\frac{P(y_r|y^{r-1})}{Q_w(y_r)}}{-\log \mu_1(w)}\Big)\bigg]\\\label{eq:gamma w 1}
&=\sum_{y_r\in \mathcal{Y}_\delta} P(y_r|y^{r-1}) \bigg( \log \frac{Q_w(y_r)}{ P(y_r|y^{r-1})}+ \log\Big(1+\frac{\log\frac{P(y_r|y^{r-1})}{Q_w(y_r)}}{-\log \mu_1(w)}\Big)\bigg)
%&\stackrel{(a)}{=} -D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q_w \Big) + \sum_{y_r} P(y_r|y^{r-1}) \log\Big(1+\frac{\log\frac{P(y_r|y^{r-1})}{Q_w(y_r)}}{-\log \mu_1(w)}\Big)
\end{align}
We bound the first term above:
\begin{align*}
&\sum_{y_r\in\mathcal{Y}} P(y_r|y^{r-1}) \log \frac{Q_w(y_r)}{ P(y_r|y^{r-1})}-\sum_{y_r\notin \mathcal{Y}_\delta} P(y_r|y^{r-1}) \log \frac{Q_w(y_r)}{ P(y_r|y^{r-1})}\\
&= D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q_w \Big) +\sum_{y_r\notin \mathcal{Y}_\delta} P(y_r|y^{r-1}) \log \frac{ P(y_r|y^{r-1})}{Q_w(y_r)}\\
&\geq D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q_w \Big) +\sum_{y_r\notin \mathcal{Y}_\delta} P(y_r|y^{r-1}) \log  P(y_r|y^{r-1})\\
&\geq D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q_w \Big) - |\mathcal{Y}| h_b(\delta),
\end{align*}
where for the last inequality we used the facts that  $p\log p \geq -h_b(p),$ and $h_b(p)\leq h_b(\delta)$ for $p\leq\delta$, and $|\mathcal{Y}_\delta|\leq |\mathcal{Y}|$.

Next, we bound the second term in \eqref{eq:gamma w 1}. The term in the logarithm is bounded as
\begin{align*}
\frac{\log\frac{P(y_r|y^{r-1})}{Q_w(y_r)}}{-\log \mu_1(w)} \geq \frac{\log P(y_r|y^{r-1}) }{-\log \mu_1(w)} > \frac{\log \delta }{-\log \mu_1(w)},
\end{align*}
where we used the fact  that $P(y_r|y^{r-1})>\delta$ as $y_r\in \mathcal{Y}_\delta$.  Therefore,  the second term in \eqref{eq:gamma w 1} is bounded as
\begin{align*}
\sum_{y_r\in \mathcal{Y}_\delta} P(y_r|y^{r-1}) \log (1+ \frac{\log \delta }{-\log \mu_1(w)})\geq \delta |\mathcal{Y}_\delta| \log (1+ \frac{\log \delta }{-\log \mu_1(w)}).
\end{align*}
We select $\delta = \sqrt{h_b^{-1}(\epsilon)}$. Since,  $\mu_1(w)\leq h_b^{-1}(\epsilon)$ for all $w\neq \wstar$, then the RHS is bounded from below as   $-|\mathcal{Y}_\delta|\sqrt{h_b^{-1}(\epsilon)}\geq -|\mathcal{Y}|\sqrt{h_b^{-1}(\epsilon)}$.

Combining the bounds for each term in \eqref{eq:gamma w 1} gives, for all $w\neq \wstar$,
% \begin{align*}
% -\Gamma(w) &\geq  D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q_w \Big) - |\mathcal{Y}|\Big( h_b(\sqrt{h_b^{-1}(\epsilon)}) +  \sqrt{h_b^{-1}(\epsilon)}\Big).
% \end{align*}
% Therefore, having $\mu_1(w)\leq h_b^{-1}(\epsilon)$ for all $w\neq \wstar$, we have that 
\begin{align}\label{eq:gamma w}
\Gamma(w) \leq D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q_w \Big) +|\mathcal{Y}|\Big( h_b\big(\sqrt{h_b^{-1}(\epsilon)}\big) +  \sqrt{h_b^{-1}(\epsilon)}\Big). 
\end{align}
Clearly the residual terms converge to zero as $\epsilon\rightarrow 0$.

Next, we consider the case $w=\wstar$. We use the Taylor's theorem for the function $f(x) = -x\log x$ around $x=1$. Hence, $f(x) = {(\log e)}\big(  (1-x) - \zeta (1-x)^2\big)$ for some $\zeta$ between $x$ and $1$. Hence, with $x= \mu_1(\Wstar)$, we have that 
\begin{align}
-\mu_1(\Wstar) \log \mu_1(\Wstar) \leq (\log e) (1-\mu_1(\wstar))-(\log e) \zeta (1-\mu_1(\wstar))^2 \leq (\log e) (1-\mu_1(\wstar)). 
\end{align}
Next, from the inequality $\log x \leq (\log e)(x-1), \forall x>0$, we have that 
\begin{align}
-\mu_1(\Wstar,y_r) \log \mu_1(\Wstar,y_r) \geq (\log e)\mu_1(\Wstar,y_r) (1- \mu_1(\Wstar,y_r)).
\end{align}
As a result of these inequalities, we have that 
\begin{align}
\Gamma(\wstar) &= \sum_{y_r} P(y_r|y^{r-1}) \log \frac{-\mu_1(\wstar)\log \mu_1(\wstar)}{-\mu_1(\wstar,y_r)\log \mu_1(\wstar,y_r)}\\
&\leq \sum_{y_r} P(y_r|y^{r-1}) \log \frac{(1-\mu_1(\wstar))}{\mu_1(\Wstar,y_r) (1- \mu_1(\Wstar,y_r))}\\\numberthis \label{eq:wstar eq1}
&=  \sum_{y_r} P(y_r|y^{r-1}) \log \frac{1-\mu_1(\wstar)}{1- \mu_1(\Wstar,y_r)}  - \sum_{y_r} P(y_r|y^{r-1}) \log \mu_1(\Wstar,y_r). 
\end{align}

We proceed with simplifying the first summation above. Using \eqref{eq:mu wstar and y}, we have that 
% \begin{equation}\label{eq:mu wstar and y}
% \mu_{1}(\Wstar, y_{r}) =\frac{\mu_1(\Wstar)Q^1_{\Wstar}(y_{r})}{P(y_r|y^{r-1}) }.
% \end{equation}
%  Therefore,
\begin{align}\label{eq:1-mu1 approximate}
(1-\mu_{1}(\Wstar, y_{r}))&=(1-\mu_1(\Wstar)) \frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)}   Q^1_{w}(y_{r})}{P(y_r|y^{r-1})}.
\end{align}
Thus, the first summation on the right-hand side of \eqref{eq:wstar eq1} is simplified as 
\begin{align*}
\sum_{y_r} P(y_r|y^{r-1}) \log \frac{P(y_r|y^{r-1})}{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)}   Q^1_{w}(y_{r})} = D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q^1_{\sim \wstar} \Big),
\end{align*}
where $Q^1_{\sim \wstar}(y_r) \deq \sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)}   Q^1_{w}(y_{r})$ for all $y_r\in \mathcal{Y}$.
Next, we bound the second summation in \eqref{eq:wstar eq1}. Using \eqref{eq:mu wstar and y}, we have that 

\begin{align*}
- \sum_{y_r} P(y_r|y^{r-1}) \log \mu_1(\Wstar,y_r)  &= -\log \mu_1(\wstar) - \sum_{y_r} P(y_r|y^{r-1}) \log \frac{Q^1_{\Wstar}(y_{r})}{P(y_r|y^{r-1}) }\\
 &= -\log \mu_1(\wstar) + D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q^1_{\wstar} \Big)\\\numberthis\label{eq:wstar eq2}
 &\leq 2 (\log e) \eta_1(\epsilon)+ D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q^1_{\wstar} \Big),
\end{align*}
where the last inequality holds from the fact that $\log x \geq (\log e) (1- \frac{1}{x})$ and that $\mu_1(\wstar)\geq 1-\eta_1(\epsilon)$, implying $$-\log \mu_1(\wstar)\leq -\log (1-\eta_1(\epsilon)) \leq (\log e) \frac{\eta_1(\epsilon)}{1-\eta_1(\epsilon)}\leq 2(\log e)\eta_1(\epsilon),$$ which holds as $\eta_1(\epsilon)\leq \frac{1}{2}$. Note that $P(\cdot|y^{r-1}) = \mu_1(\wstar)Q^1_{\wstar} + (1-\mu_1(\wstar))Q^1_{\sim \wstar}$. Therefore, from the convexity of the relative entropy, the right-hand side of \eqref{eq:wstar eq2} is bounded above by 
\begin{align*}
&~ 2(\log e)\eta_1(\epsilon) + \mu_1(\wstar) D_{KL}\Big( Q^1_{\wstar} ~\|~ Q^1_{\wstar} \Big)+(1-\mu_1(\wstar)) D_{KL}\Big( Q^1_{\sim \wstar} ~\|~ Q^1_{\wstar} \Big)\\
&\leq 2(\log e)\eta_1(\epsilon)+ \eta_1(\epsilon) D_{KL}\Big( Q^1_{\sim \wstar} ~\|~ Q^1_{\wstar} \Big)\\
& \leq (2\log e+d^{\max}) \eta_1(\epsilon),
\end{align*}
where $d^{\max}$ is the maximum of the above relative entropy for all $r\geq 1$. As a result of the above argument, we have that 
\begin{align*}
\Gamma(\wstar) &\leq D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q^1_{\sim \wstar} \Big) + (2\log e +d^{\max}) \eta_1(\epsilon)\\
&\stackrel{(a)}{\leq} \sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)}  D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q^1_{w} \Big) + (2\log e +d^{\max}) \eta_1(\epsilon)\\\numberthis\label{eq:gamma wstar}
&\stackrel{(b)}{\leq} \max_{w\neq \wstar}D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q^1_{w} \Big) + (2\log e +d^{\max}) \eta_1(\epsilon),
\end{align*}
where (a) is due to the convexity of the relative entropy on the second argument and the definition of $Q_{\sim \wstar}$. Inequality (b) follows as $\frac{\mu_1(w)}{1-\mu_1(\Wstar)}$ form a probability distribution on $w\neq \wstar$.

Combining \eqref{eq:gamma w} and \eqref{eq:gamma wstar} and \eqref{eq:log drift gamma} gives the following bound 
\begin{align}\label{eq:log drift KL 1}
\EE[\log \Htld^1_{r-1}-\log \Htld^1_{r}|\mathcal{F}_{r-1}] &\leq   \max_{w} D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q^1_{w} \Big) + \kappa(\epsilon),
\end{align}
where 
\begin{align}\label{eq:kappa}
   \kappa(\epsilon) \deq (2+d^{\max}) h_b^{-1}(\epsilon) + |\mathcal{Y}|\Big( h_b\big(\sqrt{h_b^{-1}(\epsilon)}\big) +  (1+\eta) \sqrt{h_b^{-1}(\epsilon)}\Big).
\end{align}
Observe that $\lim_{\epsilon \rightarrow 0}\kappa(\epsilon)=0$. Since $h_b(p)\leq 2\sqrt{p(1-p)}\leq 2\sqrt{p}$, then 
\begin{align*}
   \kappa(\epsilon) &\leq  (2\log e+d^{\max}) h_b^{-1}(\epsilon) + |\mathcal{Y}|(3+\eta)\sqrt{h_b^{-1}(\epsilon)}\\
   &\leq \Big(2\log e+d^{\max} + |\mathcal{Y}|(3+\eta)\Big) \sqrt{h_b^{-1}(\epsilon)}=O(\sqrt{h_b^{-1}(\epsilon)}).
\end{align*}
Note that the right-hand side of \eqref{eq:log drift KL 1} depends on the coding scheme. In what follows we remove this dependency. Note that the convexity of the relative entropy gives 
\begin{align*}
D_{KL}\Big( P(\cdot|y^{r-1})~\|~ Q^1_{w} \Big) &\leq \mu_1(\wstar) D_{KL}\Big( Q^1_{\wstar}~\|~ Q^1_{w} \Big) + (1-\mu_1(\wstar)) D_{KL}\Big( Q^1_{\sim \wstar}~\|~ Q^1_{w} \Big)\\
&\leq D_{KL}\Big( Q^1_{\wstar}~\|~ Q^1_{w} \Big)+\eta_1(\epsilon) d^{\max}.
\end{align*}

% As a result the bound in  \eqref{eq:log drift KL 1}  is simplified to the following
% \begin{align}
% \Gamma(\wstar) &\leq \max_{w} D_{KL}\Big( Q^1_{\wstar}~\|~ Q^1_{w} \Big) + 2(1+d^{\max}) \eta_1(\epsilon)
% \end{align}
% % Similarly, the bound on $\Gamma(w)$ in \eqref{eq:gamma w} is simplified to 
% \begin{align}
% \Gamma(w) &\leq D_{KL}\Big( Q^1_{\wstar}~\|~ Q^1_{w} \Big)+\eta_1(\epsilon) d^{\max}
% \end{align}

Combining the two bounds above, we simplify \eqref{eq:log drift KL 1} as 
\begin{align*}
\EE[\log \Htld^1_{r-1}-\log \Htld^1_{r}|\mathcal{F}_{r-1}] &\leq \max_{w} D_{KL}\Big( Q^1_{\wstar}~\|~ Q^1_{w} \Big) + d^{\max} \eta_1(\epsilon)+\kappa(\epsilon).
\end{align*}


We proceed by bounding the relative entropy between $Q^1_{\wstar}$ and $Q^1_{w}$ for all $w\neq \wstar$.  Let $\Qbar{1}_r = P_{Y_r|X_{1,r}, Y^{r-1}}$ which is the effective channel from the first user's perspective at time $r$. Let $\Xstar  = e_1(\Wstar, y^{r-1}).$ Then, we show that 
\begin{align}\label{eq:remove w in D}
\max_w D_{KL}\Big( Q^1_{\wstar}~\|~ Q^1_{w} \Big) \leq \max_{x_1} D_{KL}\Big(\Qbar{1}_r(\cdot | \xstar, y^{r-1})~ \|~ \Qbar{1}_r(\cdot| x_1, y^{r-1})\Big)+O(\eta_1(\epsilon)).
 \end{align} 
For the moment suppose that the above inequality holds. Then, we get the desired statement that 
\begin{align*}
\EE[\log \Htld^1_{r-1}-\log \Htld^1_{r}|\mathcal{F}_{r-1}] &\leq \max_{x_1} D_{KL}\Big(\Qbar{1}_r(\cdot | \xstar, y^{r-1})~ \|~ \Qbar{1}_r(\cdot| x_1, y^{r-1})\Big)  + O(\sqrt{h_b^{-1}(\epsilon)}).
\end{align*}
%where $\eta_2(\epsilon) = \frac{d^{\max}}{-\log \eta_1(\epsilon)} + (2+d^{\max}) \eta_1(\epsilon)$ implying that $\lim_{\epsilon\rightarrow 0} \eta_2(\epsilon)=0$.
 Repeating the above argument for $i=2,3$ completes the proof of the lemma. Hence, it remains to prove \eqref{eq:remove w in D}. 


From the convexity of the relative entropy, the left-hand side term in \eqref{eq:remove w in D} equals to 
\begin{align}\label{eq:log drift bound 1}
\max_w D_{KL}\Big( Q^1_{\wstar}~\|~ Q^1_{w} \Big) \leq \sup_{\{\mu_1(w)\}_{w\neq \wstar}}D_{KL}\Big( Q^1_{\wstar}~\|~ \sum_{w\neq \wstar}\frac{\mu_1(w)}{1-\mu_1(\wstar)} Q^1_{w} \Big),
\end{align}
where the supremum is taken over all distributions $\mu_1(\cdot)$ on all $w\neq \wstar$ satisfying $\mu_1(w)\geq 0$ and $\sum_{w\neq \wstar} \mu_1(w) = 1-\mu_1(\wstar)$.
%\begin{align}
%D_{KL}\Big( Q^1_{\wstar}~\|~ Q^1_{w} \Big)  = \sum_{y_r} Q^1_{\wstar}(y_r) \log \frac{Q^1_{\wstar}(y_r) }{Q^1_{w}(y_r) }.
%\end{align}
We provide an upper bound on the right-hand side of \eqref{eq:log drift bound 1} by approximating $Q^1_{\wstar}(y_r)$ and by bounding $\sum_{w\neq \wstar}\frac{\mu_1(w)}{1-\mu_1(\wstar)} Q^1_{w}$ from below. 



%We start with bounding $Q^1_{w}(y_r)$. Suppose $x_1 = e_1(w, y^{r-1})$. By $\mathcal{E}_1^{-1}(x_1)$ denote all $w\in [1:M_1]$ that mapped to $x_1$, that is $ e_1(w, y^{r-1})= x_1$. By definition 
%\begin{align*}
%v_1(x_1) \deq \prob{X_{1,r} = x_1 | y^{r-1}} = \prob{W_1 \in \mathcal{E}_1^{-1}(x_1) | y^{r-1}} = \sum_{w\in \mathcal{E}_1^{-1}(x_1)} \mu_1(w).
%\end{align*}
%Also, note that 
%\begin{align*}
%\Qbar(y_r| x_1, y^{r-1}) &\deq \prob{Y_r = y_r| y^{r-1}, X_{1,r}=x_1}\\
%&= \sum_{w\in \mathcal{E}_1^{-1}(x_1)} \prob{W_1=w, Y_r = y_r| y^{r-1}, X_{1,r}=x_1}\\
%&=\sum_{w\in \mathcal{E}_1^{-1}(x_1)} \prob{W_1=w| y^{r-1}, X_{1,r}=x_1} Q^1_w(y_r)\\
%& = \sum_{w\in \mathcal{E}_1^{-1}(x_1)} \frac{\mu_1(w)}{v_1(x_1)} Q^1_w(y_r)
%\end{align*}

We start with bounding the second term from below. For any $x_1\in\mathcal{X}_1$, define $\nu_1(x_1) \deq \prob{X_{1,r}=x_1 | y^{r-1}}$.
Then, for any choice of $\mu_1(w), w\neq \wstar$, we have that
 \begin{align*}
&\sum_{w \notin \Wstar } \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(y_r) =  \frac{1}{1-\mu_1(\Wstar)}\sum_{w \notin \Wstar} \prob{W_1= w, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& \stackrel{(a)}{=} \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{w \notin  \wstar,\\ x_1\notin  \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{W_1= w, X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }+\kappa'\\
& \stackrel{(b)}{=} \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{w\\ x_1 \notin \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{W_1= w, X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }+\kappa'\\
& =\frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{x_1 \notin  \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }+\kappa'\\
& = \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{x_1\notin \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{X_{1,r} = x_1, X_{2,r} = x_2\big|~Y^{r-1}= y^{r-1} }Q(y_r | x_1,x_2)+\kappa'\\
& \stackrel{(c)}{=} \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{x_1\notin  \xstar}} \prob{X_{1,r} = x_1 \big|~Y^{r-1}= y^{r-1} } \sum_{x_2\in\mathcal{X}_2} \prob{X_{2,r} = x_2\big|~Y^{r-1}= y^{r-1},X_{1,r} = x_1 } Q(y_r | x_1,x_2)+\kappa'\\\numberthis \label{eq:Q1 Qbar bound 2}
&\stackrel{(d)}{=} \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{x_1\notin  \xstar}} \nu_1(x_1) \Qbar{1}_r(y_r|x_1, y^{r-1})+\kappa'%\\\numberthis \label{eq:Q1 Qbar bound 2}
%& \stackrel{(e)}{\approx} \frac{1}{1-\nu_1(\xstar)}\sum_{\substack{x_1\notin  \xstar}} \nu_1(x_1) \Qbar{1}_r(y_r|x_1, y^{r-1}),
 \end{align*}
 where (a) follows by defining
 \begin{align*}
     \kappa'\deq \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{w \notin  \wstar,\\ x_1= \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{W_1= w, X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1}} 
 \end{align*} 
 and by summing over $x_1$ and $x_2$. %Note that this is an inequality because the summation is not over all values of $x_1$. 
 Equality (b) holds by removing the condition $w\neq \wstar$. This is an equality, because the probability of the event $\{W_1 =\wstar, X_{1,r} \neq \xstar\}$ is zero. Equality (c) follows by breaking the joint probability on $(X_{1,r}, X_{2,r})$ and further moving the summation on $x_2$. Equality (d) is due to the definition of $\nu_1$ and $\Qbar{1}_r$. %Lastly, (e) is due to the fact that $\nu_1(\xstar) \approx \mu_1(\wstar) \approx 1-\eta_1(\epsilon)$. 
 
 


 Next, we approximate $Q^1_{\wstar}(y_r)$ by deriving a lower bound and an upper bound that are converging to each other. We start with the lower bound on $Q^1_{\wstar}(y_{r})$. Since $X_{1,r}=e_1(W_1, Y^{r-1}),$  we have that 
\begin{align*}
Q^1_{\wstar}(y_{r}) &= \prob{Y_r = y_r \big|~ W_1 =  \wstar, Y^{r-1}=y^{r-1}, X_{1,r} =  \xstar}\\
&= \sum_{x_2 \in\mathcal{X}_2} \prob{Y_r = y_r, X_{2,r} = x_2 \big|~ W_1 = \wstar, Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\\numberthis \label{eq:Q1 Qbar eq 1}
&= \sum_{x_2 \in\mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~ W_1 = \wstar, Y^{r-1}=y^{r-1}, X_{1,r} = \xstar }Q(y_r| x_2, \xstar)
%&= \sum_{x_2 \in\mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} = \xstar }\frac{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar, X_{2,r} = x_2\}}{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar\}}Q(y_r| x_2, \xstar),
\end{align*}
where the last equality holds as the channel is memoryless.  Next, we bound the conditional probability on $X_{2,r}$ in the above summation. This quantity equals to 
 \begin{align}\label{eq:Q1 Qbar eq 2}
 \prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} = \xstar }\frac{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar, X_{2,r} = x_2\}}{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar\}}.
 \end{align}
 The denominator is greater than $(1-\eta_1(\epsilon))$ because of the following argument: 
 \begin{align*}
\prob{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} &= \frac{\PP\{W_1= \wstar, X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}{\PP\{X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}\\
 &= \frac{\PP\{W_1= \wstar| Y^{r-1}=y^{r-1}\}}{\PP\{X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}\\
 &= \frac{\mu_1(\wstar)}{\PP\{X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}\\
 &\geq 1-\eta_1(\epsilon),
 \end{align*}
 where the last inequality holds as the denominator is less than one and that $\mu_1(\wstar)\geq 1-\eta_1(\epsilon).$ 
%  Hence, from \eqref{eq:Q1 Qbar eq 2}, we have that
% \begin{align*}
% \frac{1}{1-\eta_1(\epsilon)}\prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} = \xstar }
%  \end{align*} 
 Hence, from  \eqref{eq:Q1 Qbar eq 1}, we have that 
  \begin{align*}
Q^1_{\wstar}(y_{r}) & \leq \frac{1}{1-\eta_1(\epsilon)}\sum_{x_2 \in \mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} = \xstar } Q(y_r| x_2, \xstar)\\\numberthis \label{eq:Q1 Qbar bound 1}
& = \frac{1}{1-\eta_1(\epsilon)} \Qbar{1}_r(y_r| \xstar, y^{r-1}).
 \end{align*}
 
With the bounds in \eqref{eq:Q1 Qbar bound 1} and \eqref{eq:Q1 Qbar bound 2}, the right-hand side of \eqref{eq:log drift bound 1} is bounded as 
 \begin{align*}
 D_{KL}\Big( Q^1_{\wstar}~\|~ \sum_{w\neq \wstar}\frac{\mu_1(w)}{1-\mu_1(\wstar)} Q^1_{w}& \Big)  =  \sum_{y_r}Q^1_{\Wstar}(y_{r}) \log \frac{Q^1_{\Wstar}(y_{r})}{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(y_{r})}\\
&\stackrel{(a)}{\leq}  \sum_{y_r}Q^1_{\Wstar}(y_{r}) \log \frac{\frac{1}{1-\eta_1(\epsilon)}\Qbar{1}_r(y_{r}|\xstar, y^{r-1})}{\sum_{x_1\notin \xstar} \frac{\nu_1(x_1)}{1-\mu_1(\wstar)} \Qbar{1}_r(y_{r}|x_1, y^{r-1})}\\
&\stackrel{(b)}{\leq} \sum_{y_r}\Qbar{1}_r(y_{r}|\xstar, y^{r-1}) \log \frac{\Qbar{1}_r(y_{r}|\xstar, y^{r-1})}{\sum_{x_1\notin \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar{1}_r(y_{r}|x_1, y^{r-1})}-\log (1-\eta_1(\epsilon))\\\numberthis\label{eq:log drift bound 2}
& = D_{KL}\Big(\Qbar{1}_r(\cdot | \xstar, y^{r-1})|| \sum_{x_1\neq \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar{1}_r(\cdot| x_1, y^{r-1})\Big)+O(\eta_1(\epsilon)),
 \end{align*}
 where (a) follows from \eqref{eq:Q1 Qbar bound 1} and \eqref{eq:Q1 Qbar bound 2}, and (b) follows from the following argument for bounding $Q^1_{\wstar}(y_{r})$ from below: 
\begin{align*}
Q^1_{\wstar}(y_{r}) &= \prob{Y_r = y_r \big|~ W_1 = \wstar, Y^{r-1}=y^{r-1}, X_{1,r}= \xstar}\\
%&= \frac{\prob{Y_r = y_r, W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}}{\prob{W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}}\\
& \geq \prob{Y_r = y_r, W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
& = \prob{Y_r = y_r \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} \prob{ W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar, Y_r = y_r}\\
&=\Qbar{1}_r(y_r|\xstar, y^{r-1}) \frac{\prob{ W_1 = \wstar, X_{1,r} = \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}{\prob{X_{1,r} = \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}\\
&\stackrel{(a)}{=}\Qbar{1}_r(y_r|\xstar, y^{r-1}) \frac{\prob{ W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}{\prob{X_{1,r}= \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}\\
&\stackrel{(b)}{=} \Qbar{1}_r(y_r|\xstar, y^{r-1})\prob{ W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}\\
& \stackrel{(c)}{=} \Qbar{1}_r(y_r|\xstar, y^{r-1}) \mu_1(\wstar, y_r),\\\numberthis\label{eq:Q1 Qbar bound 3}
& \stackrel{(d)}{\geq} \Qbar{1}_r(y_r|\xstar, y^{r-1})(1-\eta_2(\epsilon))
%
%& = \sum_{w}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} - \sum_{w\neq \wstar}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%& = \prob{Y_r = y_r \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} - \sum_{w\neq \wstar}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%& = \Qbar{1}_r(y_r|\xstar, y^{r-1}) - \prob{Y_r = y_r, W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\\numberthis\label{eq:log drift bound 2}
%& \geq \Qbar{1}_r(y_r|\xstar, y^{r-1}) - \prob{W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}
 \end{align*} 
where  (a) holds as $X_{1,r}$ is a function of $(W_1, Y^{r-1})$, (b) holds as the denominator is less than one, (c) is due to the definition of $\mu_1(w_1, y_r)$, and (d) holds from \eqref{eq:1-mu1 approximate} and by defining 
\begin{align*}
\eta_2(\epsilon) =\eta_1(\epsilon)\frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)}   Q^1_{w}(y_{r})}{P(y_r|y^{r-1})}.
\end{align*}
 Lastly, by taking the supermum of \eqref{eq:log drift bound 2} over $\nu_1(x_1), x_1\neq \xstar$, we obtain the desired bound in \eqref{eq:remove w in D}. With that the proof is complete.
%\begin{align*}
%\prob{Y_r = y_r, W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} & = \frac{\prob{Y_r = y_r, W_1 \neq \wstar, X_{1,r} = \xstar \big|~ Y^{r-1}=y^{r-1}}}{\prob{X_{1,r} = \xstar \big|~ Y^{r-1}=y^{r-1}}}\\
%& \leq \frac{\prob{W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}}}{\nu_1(\xstar)}\\
%& \leq \frac{\epsilon'}{\nu_1(\xstar)}\\
%&\leq \frac{\epsilon'}{1-\epsilon'}
% \end{align*} 
 
\end{IEEEproof}


==> proofs/Proof_thm_upperbound_Berline.tex <==
\subsection{Proof of the Upper-Bound}\label{subsec: proof of theorem}
Consider any $(N, M_1,M_2)$ VLC with probability of error $P_e$, and stopping time $T$. Suppose the message at Encoder 2, $W_2$, is made available to all terminals. For the new setup, as $W_2$ is available at the Decoder, the average probability of error is $P_e^1 \triangleq P\{\hat{W}_1\neq W_1\}$. Note that $P_e\geq P_e^1$. We refer to such setup as $W_2$-assisted MAC. For a maximum a \textit{posteriori} decoder, after $n$ uses of the channel and assuming the realization $Y^n=y^n$ and $W_2=w_2$, define
\begin{align*}
T_1^{\delta} \triangleq \inf \big\{n: \max_{1\leq i \leq M_1} P(W_1=i| y^n, w_2)\geq 1-\delta \big \},
\end{align*}
where $\delta>0$ is a fixed real number. Also, let $\tau_1 \triangleq \min  \{ T, T_1^{\delta}\}$. Note that $\tau_1$ is a stopping time w.r.t the filtration $\{\mathcal{F}_{W_2}\times \mathcal{F}_t\}_{t>0}$. The following lemma provides a lower-bound on the probability of error for such setup. 

\begin{lem}\label{lem: hypothesis gini-aided MAC}
The probability of error, $P_e$, for a hypothesis testing over a $W_2$-assisted MAC and variable length codes satisfies the following inequality 
\begin{align*}
P_e\geq \frac{\min \{P(H), P(H^c)\}}{4}e^{-D_1\EE[T]},
\end{align*}  
where $\{H, H^c\}$ are the two hypothesizes and $T$ is the stopping time of the variable length code. 
\end{lem}

\begin{lem}\label{lem: zeta}
For a given MAC with finite $D_3$ the following holds
\begin{align*}
\zeta p(w_1, w_2|y^{n-1})\leq  p(w_1, w_2|y^{n})\leq \frac{ p(w_1, w_2|y^{n-1})}{\zeta},
\end{align*}
where $\zeta\triangleq \min_{x_1,x_2,y} Q(y|x_1,x_2)$.
\end{lem}
%\begin{proof}
The above lemmas are extensions of Lemma 1 and Proposition 2 in \cite{Berlin} for MAC. The proofs follow from similar arguments and are omitted.
%\end{IEEEproof}

\begin{lem}\label{lem: P_e lowerbound W_2 assisted MAC}
Given a MAC with $D_3<\infty$, and for any $(N, M_1,M_2)$ VLC with probability of error $P_e$ the following holds
\begin{align}\label{eq: P_e^1}
P_e \geq \frac{\zeta \delta}{4} e^{-D_1 \EE[T- \tau_1]},
\end{align}
where $\zeta\triangleq \min_{x_1,x_2,y} Q(y|x_1,x_2)$.
\end{lem} 

\begin{IEEEproof}
Suppose the VLC is used for a $W_2$-assisted MAC. As discussed before, $P_e\geq P_e^1$. 
%
% Since $W_2$ is available at all terminals, $\tau_1$ can be calculated both at Encoder 1 and  the Decoder. Let $$P_e^1(y^n, w_2)\triangleq 1-\max_{1\leq i \leq M_1} P(W_1=i| y^n, w_2).$$ 
We modify the encoding and the decoding functions of the VLC used for the MAC. Let $\mathcal{H}_1 \subseteq \mathcal{M}_1$ be a subset of the message set $\mathcal{M}_1$.  The subset $\mathcal{H}_1$ is to be determined at time $\tau_1$. The new decoding function, at time $T$, decides whether the message belongs to $\mathcal{H}_1$. The new encoding functions are the same as the original one until the time $\tau_1$. Then, after $\tau_1$, the transmitters perform a VLC to resolve the binary hypothesis  $\{W_1\in \mathcal{H}_1\}$ and $\{W_1\notin \mathcal{H}_1\}$. This hypothesis problem is performed from $\tau_1$ to $T$. With these modifications, the error probability of this binary hypothesis problem is a lower-bound on $P_e$.  In what follows, we present a construction for $\mathcal{H}_1$. Then, we apply Lemma \ref{lem: hypothesis gini-aided MAC} to complete the proof. 

Let $P_e^1(y^n, w_2)\triangleq 1-\max_{1\leq i \leq M_1} P(W_1=i| y^n, w_2).$ 
 The quantity $P_e^1(y^{\tau_1}, w_2)$ can be calculated at all terminals. 
  By definition, at time $\tau_1-1$, the inequality $P(W_1=i| Y^{\tau_1-1}, W_2)<1-\delta$ holds almost surely for all $i\in [1:M_1]$.  This implies that $P_e^1(Y^{\tau_1-1}, W_2)>\delta$. Hence, by Lemma \ref{lem: zeta}  at time $\tau_1$ the inequality $P_e^1(Y^{\tau_1},W_2)\geq \zeta \delta$ holds almost surely.  We consider two cases $P_e^1(y^{\tau_1}, w_2)\leq \delta$ and $P_e^1(y^{\tau_1}, w_2)>\delta$, where $\delta$ is the constant used in the definition of $T_1^{\delta}$.  For the first case,  $\mathcal{H}_1$ is the set consisting of the message with the highest a \textit{posteriori} probability. Since $P_e^1(y^{\tau_1}, w_2)\leq \delta$, then $P(\mathcal{H}_1)\geq 1-\delta$. In addition, as $P_e^1(y^{\tau_1}, w_2)\geq \zeta \delta$, then $P(\mathcal{H}^c_1)>\zeta \delta$. For the second case, set $\mathcal{H}_1$ to be a set of messages such that $P(\mathcal{H}_1)>\delta/2$ and $P(\mathcal{H}_1)<1-\delta$. Such set exists, since $P(W_1=i| Y^{\tau-1}, W_2)<1-\delta$ holds for all messages $i\in [1:M_1]$.

Note that by the above construction, for each case, $P(\mathcal{H}_1) \in [\zeta \delta, 1-\zeta\delta] $. Thus, from Lemma \ref{lem: hypothesis gini-aided MAC} and the argument above, the inequality 
\begin{align*}
P\{\hat{W}_1\neq W_1|Y^{\tau},W_2\} \geq \frac{\zeta \delta}{4} e^{-D_1 \EE[T- \tau|Y^{\tau}, W_2]}
\end{align*}
holds almost surely. Next, we take the expectation of the above expression. The lemma follows by the convexity of $e^{-x}$ and Jensen's inequality. 

\end{IEEEproof}
Next, we apply the same argument for the case where $W_1$ is available at all the terminals. For that define
\begin{align*}
T_2^{\delta}&\triangleq \inf \big\{n: \max_{1\leq j \leq M_2} P(W_2=j| y^n, w_1)\geq 1-\delta \big \},
%P_e^2 &\triangleq P\{\hat{W}_2\neq W_2\}
\end{align*}
and let $\tau_2 \triangleq \min  \{ T, T_2^{\delta}\}$. By symmetry, Lemma \ref{lem: P_e lowerbound W_2 assisted MAC} holds for this case and we obtain
\begin{align}\label{eq: P_e^2}
P_e \geq \frac{\zeta \delta}{4} e^{-D_2 \EE[T- \tau_2]}.
\end{align}
%Next, define $P_e^3(y^n)=P(\hat{W}_1\neq W_1, \hat{W}_2\neq W_2|y^n)$ and let $P_e^3=\EE[P_3^3(Y^T)]$. Hence, $P_e^3\leq P_e$. 
Next, define the following stopping times:
\begin{align*}
T_3^{\delta}&\triangleq \inf \big\{n: \max_{i,j} P(W_1=i, W_2=j| y^n)\geq 1-\delta \big \}.
%\tau_3 &\triangleq \min  \{ T, T_3^{\delta}\}.
%
%T_3 \triangleq \min \{n: P_e^3(y^n)\leq \delta\}
\end{align*}
Also, let $\tau_3=\min\{T, T_3^{\delta}\}$. using a similar argument as in the above, we can show that 
\begin{align}\label{eq: P_e^3}
P_e \geq \frac{\zeta \delta}{4} e^{-D_3 \EE[T- \tau_3]}.
\end{align}
For that, after time $\tau_3$, we formulate a binary hypothesis problem in which the transmitters determine whether $(W_1,W_2)\in \mathcal{H}_3$ or not. Here, $\mathcal{H}_3$ is a subset which is constructed using a similar method as for $\mathcal{H}_1$ in the proof of Lemma \ref{lem: P_e lowerbound W_2 assisted MAC}.  We further allow the transmitters to communicate with each other after $\tau_3$. 
The maximum of the right-hand sides of \eqref{eq: P_e^1}, \eqref{eq: P_e^2} and \eqref{eq: P_e^3} gives a lower-bound on $P_e$. The lower-bound depends on the expectation of the stopping times $\tau_i, i=1,2,3$. In what follows, we provide a lower-bound on $\EE[\tau_i]$. 
%\begin{align}\label{eq: P_e }
%P_e \geq \frac{\zeta \delta}{4} e^{-D_i \EE[T- \tau_i]}, \quad i=1,2,3.
%\end{align}
 Define the following random processes.
 \begin{equation*}
 \begin{aligned}[c]
H^1_t&\triangleq H(W_1|~\mathcal{F}_{W_2}\times \mathcal{F}_t),\\ 
H^2_t &\triangleq H(W_2|~\mathcal{F}_{W_1}\times \mathcal{F}_t),\\
H^3_t&\triangleq H(W_1,W_2|~ \mathcal{F}_t),
\end{aligned}
 \end{equation*}
\begin{lem}\label{lem: linear drift MAC FB}
Given a $(M_1, M_2, N)$-VLC, for any $\epsilon>0$ there exist $L$ and a probability distribution $P_{X_1^LX_2^LY^L}$ that factors as in \eqref{eq: factorization of P} such that 
the following inequalities hold almost surely for $1 \leq t \leq N$
\begin{align*}
\EE[H^1_{t+1}-H^1_{t}|\mathcal{F}_{W_2}\times \mathcal{F}_t] & \geq - (I^1_L+\epsilon), \\
\EE[H^2_{t+1}-H^2_{t}|\mathcal{F}_{W_1}\times \mathcal{F}_t] & \geq - (I^2_L+\epsilon),\\
\EE[H^3_{t+1}-H^3_{t}|\mathcal{F}_t] & \geq - (I^3_L+\epsilon).
\end{align*}
where $i=1,2,3$, and $I_L^i$ is defined as in \eqref{eq: I_L^1}-\eqref{eq: I_L^3}.
\end{lem}
\begin{IEEEproof}
The proof is provided in Appendix \ref{appx: proof of lem linear drift}.
\end{IEEEproof}
We need the following lemma to proceed. The lemma is a result of Lemma 4 in \cite{Burnashev}, and we omit its proof.
\begin{lem}\label{lem: H_t+1 - H_tis bounded}
For any $t\geq 1$ and $i=1,2,3$, the following inequality holds almost surely w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2} \times \mathcal{F}_t$
\begin{align*}
\log H_t^i-\log H_{t+1}^i \leq \max_{\substack{j,l\in [1:M_1]\\ k,m\in [1:M_2]}}\max_{y\in \mathcal{Y}} \frac{\hat{Q}_{j,k}(y)}{\hat{Q}_{l,m}(y)}.
\end{align*}
\end{lem}

From Lemma \ref{lem: linear drift MAC FB} and the fact that $H_t^i\leq \log_2 M_i < \infty$, the processes $\{H_t^i+ (I_L^1+\epsilon)t\}_{t>0}$ are submartingales for $i=1,2,3$. In addition, from Lemma \ref{lem: H_t+1 - H_tis bounded} and the inequalities $\EE[\tau_i]\leq \EE[T]\leq N <\infty$, we can apply Doob's Optional Stopping Theorem for each submartingale $\{H_t^i+ (I_L^1+\epsilon)t\}_{t>0}$. Then, we get:
\begin{align}\label{eq: bound on log M_i for MAC Exp}
\log M_i &\leq \EE[H^i_{\tau_i}]+\EE[\tau_i] (I_L^i+\epsilon)
%&\leq h_b(\delta)+\EE[\tau] (I_L^i+\epsilon),
\end{align}
where $M_3=M_1 M_2$.

\begin{lem}
The following inequality holds for each $i=1,2,3$
\begin{align*}
\EE[H^i_{\tau_i}]\leq h_b(\delta)+(\delta+\frac{P_e}{\delta})\log_2 M_i.
\end{align*}
\end{lem}
\begin{IEEEproof}
We prove the lemma for the case $i=1$. The proof for $i=2,3$ follows from a similar argument. For $i=1$, we obtain 
\begin{align}\nonumber
\EE[H_{\tau_1}^1]&=P\{P_e(Y^{\tau_1},W_2)>\delta\}\EE[H_{\tau_1}^i|P_e(Y^{\tau_1},W_2)>\delta]+P\{P_e(Y^{\tau_1},W_2)\leq \delta\}\EE[H_{\tau_1}^1|P_e(Y^{\tau_1},W_2)\leq \delta]\\\label{eq: bound on EE H_tau_i}
&\leq P\{P_e(Y^{\tau_1},W_2)>\delta\}\log_2 M_1 + P\{P_e(Y^{\tau_1},W_2)\leq \delta\}\EE[H_{\tau_1}^i|P_e(Y^{\tau_1},W_2)\leq \delta].
\end{align}

Note that the event $\{P_e(Y^{\tau_1},W_2)>\delta\}$ implies that $\tau_1=T$, and $P_e(y^{\tau_1},W_2)>\delta$ for all $0\leq n \leq T$. Hence, this event is included in the event $\{P_e(Y^{T},W_2)>\delta\}$. Thus, applying Markov inequality gives 
\begin{align*}
P\{P_e(Y^{\tau_1},W_2)>\delta\}\leq P\{P_e(Y^{T},W_2)>\delta\} \leq \frac{P_e}{\delta}.
\end{align*}
As a result of the above argument, the right-hand side of \eqref{eq: bound on EE H_tau_i} does not exceed the following 
 \begin{align*}
 \frac{P_e}{\delta} \log_2 M_1 + \EE[H_{\tau_1}^1|P_e(Y^{\tau_1},W_2)\leq \delta].
 \end{align*}
 From Fano's inequality we obtain 
\begin{align*}
\EE[H_{\tau_1}^1 | P_e(Y^{\tau_1},W_2)\leq \delta]\leq h_b(\delta)+\delta \log_2 M_1.
\end{align*}
The proof is complete from the above inequality.
\end{IEEEproof}
 As a result of the above lemma and \eqref{eq: bound on log M_i for MAC Exp}, the inequality  $\EE[\tau_i]\geq \frac{\log M_i}{I_L^i+\epsilon}-\frac{h_b(\delta)}{I_L^i+\epsilon}$ holds. Finally, combining this inequality with \eqref{eq: P_e^1}-\eqref{eq: P_e^3} completes the proof of the theorem.
  

==> proofs/Proof_thm_upperbound_Burnashev.tex <==
\subsection{An Alternative Proof for the Upper-Bound}\label{subsec: proof of theorem Burnashev}

 
In this part of the paper, we provide a series of Lemmas that are used to prove the Theorem. % The proof is given in Appendix \ref{appx: proof of thm Error Exp Upper bound}. 
 Define the following random processes.
%\begin{align*}
%\Pi_1(i|j)\triangleq P(W_1=i|W_2=j, \mathcal{F}_t)\\
%\Pi_2(i|j)\triangleq P(W_2=i|W_1=j, \mathcal{F}_t)\\
%\Pi_3(i,j)\triangleq P(W_1=i,W_2=j, \mathcal{F}_t)
%\end{align*}
%\begin{align*}
%H^1_t&\triangleq H(W_1|~\mathcal{F}_{W_2}\times \mathcal{F}_t),\\
%H^2_t &\triangleq H(W_2|~\mathcal{F}_{W_1}\times \mathcal{F}_t),\\
%H^3_t&\triangleq H(W_1,W_2|~ \mathcal{F}_t).
%\end{align*}
% \begin{equation*}
% \begin{aligned}[c]
%H^1_t&\triangleq H(W_1|~\mathcal{F}_{W_2}\times \mathcal{F}_t),\\
%H^3_t&\triangleq H(W_1,W_2|~ \mathcal{F}_t), \quad 
%\end{aligned}
%\quad
%\begin{aligned}[c]
%H^2_t &\triangleq H(W_2|~\mathcal{F}_{W_1}\times \mathcal{F}_t),\\
%t&\in \NN.
%\end{aligned}
% \end{equation*}
%
%For three numbers $\lambda_1, \lambda_2, \lambda_3$, satisfying $\lambda_i \geq 0$, $\lambda_1+\lambda_2+\lambda_3=1$, define $H_t(\underline{\lambda})\triangleq \lambda_1 H_t^1 + \lambda_2 H_t^2+\lambda_3 H_t^3$.
%From the properties of conditional entropy, $H_t^3 \geq H_t^i,$ where $t\geq 0, i=1,2$. 

\begin{lem}\label{lem: generalized fano for MAC-FB}
For an $(M_1, M_2, N)$-VLC with probability of error $P_e$ the following inequality holds
\begin{align*}
\EE[H^i_T]\leq h_b(P_e)+P_e \log_2(M_1M_2-1), \quad \text{for} \quad  i=1,2,3.
\end{align*}
\end{lem}

\begin{IEEEproof}
The proof follows from Fano's Lemma as in \cite{Burnashev}.
\end{IEEEproof}
%
%\begin{lem}
%For $t\geq 1$, and $\lambda_i >0, i=1,2,3, \lambda_1+\lambda_2+\lambda_3=1$ the following inequalities hold
%\begin{align*}
%\EE[H_{t+1}(\underline{\lambda})-H_{t}(\underline{\lambda})] \geq -C(\underline{\lambda}),
%\end{align*}
%where $C(\underline{\lambda})$ is the intersection of the line $\underline{\lambda}. \underline{R}$ and the boundary of the capacity region.
%\end{lem}

%In the next two lemmas, we provide bounds on the rate of decrease of the entropies $H_t^1, H_t^2, H_t^3$. 
%\begin{lem}\label{lem: linear drift MAC FB}
%Given an $(M_1, M_2, N)$-VLC and for any $\epsilon>0$, there exist $L$ and a probability distribution $P_{X_1^LX_2^LY^L}$ that factors as in \eqref{eq: factorization of P} such that 
%the following inequalities hold almost surely for $1 \leq t \leq N$
%\begin{align*}
%\EE[H^1_{t+1}-H^1_{t}|\mathcal{F}_{W_2}\times \mathcal{F}_t] & \geq - (I^1_L+\epsilon), \\
%\EE[H^2_{t+1}-H^2_{t}|\mathcal{F}_{W_1}\times \mathcal{F}_t] & \geq - (I^2_L+\epsilon),\\
%\EE[H^3_{t+1}-H^3_{t}|\mathcal{F}_t] & \geq - (I^3_L+\epsilon).
%\end{align*}
%where $i=1,2,3$, and $I_L^i$ is defined as in \eqref{eq: I_L^1}-\eqref{eq: I_L^3}.
%\end{lem}
%\begin{IEEEproof}
%The proof is given in Appendix \ref{appx: proof of lem linear drift}.
%\end{IEEEproof}



\begin{lem}\label{lem: log drift MAC-FB}
There exists $\epsilon>0$ such that, if $H_t^i \leq \epsilon$, then 
\begin{align*}
\EE[\log H_{t+1}^1-\log H^1_{t}|\mathcal{F}_{W_2}\times\mathcal{F}_t] &\geq -(D_1+\epsilon),\\
\EE[\log H_{t+1}^2-\log H^2_{t}|\mathcal{F}_{W_1}\times \mathcal{F}_t] &\geq -(D_2+\epsilon),\\
\EE[\log H_{t+1}^3-\log H^3_{t}|\mathcal{F}_t] &\geq -(D_3+\epsilon)
\end{align*}
holds almost surely, where $D_i, i=1,2,3$ are defined in \eqref{eq: definiton of D_i}.
\end{lem}
\begin{IEEEproof}
The proof is given in Appendix \ref{appx: proof of lem log drift}.
\end{IEEEproof}

%We need the following lemma to proceed. The lemma is a result of Lemma 4 in \cite{Burnashev}, and we omit its proof.
%
%\begin{lem}
%For any $t\geq 1$ and $i=1,2,3$, the following inequality holds almost surely w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2} \times \mathcal{F}_t$
%\begin{align*}
%\log H_t^i-\log H_{t+1}^i \leq \max_{\substack{j,l\in [1:M_1]\\ k,m\in [1:M_2]}}\max_{y\in \mathcal{Y}} \frac{\hat{Q}_{j,k}(y)}{\hat{Q}_{l,m}(y)}.
%\end{align*}
%\end{lem}
%We can show that the constant $K$ in the lemma is $$K=\max_{\substack{j,l\in [1:M_1]\\ k,m\in [1:M_2]}}\max_{y\in \mathcal{Y}} \frac{\hat{Q}_{j,k}(y)}{\hat{Q}_{l,m}(y)}.$$

\begin{lem}\label{lem: Z_i are submartingale}
For $i=1,2,3$, define  random process $\{Z^{(i)}_t\}_{t\geq 1}$ as 
\begin{align}\nonumber
Z^{(i)}_t =&\left(\frac{\log H^i_t-\log \epsilon}{D_i}+t+f_i(\log \frac{H^i_t}{\epsilon})\right)\mathbbm{1}{\{H^i_t \leq \epsilon\}}\\\label{eq: Z_t^i}
&+ \left(\frac{H^i_t-\epsilon}{I^i_L}+t\right)\mathbbm{1}{\{H^i_t \geq \epsilon	\}}
\end{align} 
where the function $f_i$ is defined as $f_i(y)=\frac{1-e^{-\mu_i y}}{D_i \mu_i}.$ Then, there exists $\mu_i>0$ such that $Z^{(i)}_t$ is a submartingale w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2}\times\mathcal{F}_t$.
\end{lem}
\begin{IEEEproof}[Outline of the proof]
Suppose $W_2=m$ for some $m\in [1:M_2]$. Given this event and using the same argument as in the proof of Theorem 1 in \cite{Burnashev} we can show that $Z_{t}^{(i)}| W_2=m$ is a submartingale for all $m$. More precisely, the inequality
\begin{align*}
\EE\{Z_{t}^{(i)}-Z_{t+1}^{(i)}| \mathcal{F}_{W_1}\times \mathcal{F}_{W_2}\}\leq 0,
\end{align*} 
holds almost surely w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2}$. Taking the expectation of the both sides in the above inequality gives
\begin{align*}
\EE\{Z_{t}^{(i)}-Z_{t+1}^{(i)}\}\leq 0,\quad \forall t\geq 0, ~ i=1,2,3.
\end{align*}
Thus, $Z_{t}^{(i)}$ is a submartingale for $i=1,2,3$ and w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2}\times \mathcal{F}_t$.
\end{IEEEproof}


%\begin{corollary}
%Suppose  $\alpha_1, \alpha_2, \alpha_3$ are non-negative numbers such that $\alpha_1+\alpha_2+\alpha_3=1$. Define $Z_t = \alpha_1 Z_t^{(1)}+\alpha_2 Z_t^{(2)}+\alpha_3 Z_t^{(3)}$. Then, $Z_t$ is a submartingale w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2}\times\mathcal{F}_t$.  
%\end{corollary}
%\red{[AA: this corollary is NEVER used in the proof and we can delete it.]}

The Theorem follows from the above lemma, and the proof is given in Appendix \ref{appx: proof of thm Error Exp Upper bound}.



==> proofs/lmmas_proof.tex <==
{
\section{Proof of Lemma \ref{lem: linear drift MAC FB}}\label{appx: proof of lem linear drift}
\begin{IEEEproof}
%We prove the lemma for the case when $i=1$. The proof for $i=2,3$ follows using a similar argument.  
Given $Y^t=y^t, W_1=m_1, W_2=m_2$, we obtain 
\begin{align}\nonumber
\EE[& H^1_{t+1}-H^1_{t}|m_2, y^t ]\\\nonumber
&= -I(W_1;Y_{t+1}|m_2, y^t )\\\nonumber
&= -I(W_1;Y_{t+1}|m_2,  x_{2}^{t+1}, y^t )\\\nonumber
&=-H(Y_{t+1}|m_2, x_{2}^{t+1}, y^t )+H(Y_{t+1}|m_2, x_{2}^{t+1},W_1, y^t)\\ \nonumber
&=-H(Y_{t+1}|m_2, x_{2}^{t+1}, y^t )\\\nonumber
& \quad +H(Y_{t+1}|m_2, x_{2}^{t+1},W_1, X_{1}^{t+1}, y^t)\\\nonumber
&\stackrel{(a)}{=}-H(Y_{t+1}|m_2, x_{2}^{t+1}, y^t )  +H(Y_{t+1}|x_{2}^{t+1}, X_{1}^{t+1},y^t)
\label{eq: bound on linear drift of H^1 }\\
&\triangleq -J^1_{t+1}(m_2,x_{2}^{t+1},y^t)
\end{align}
where $(a)$ follows because condition on the channel inputs $X_{1, t+1}, X_{2, t+1}$, the output $Y_{t+1}$ is independent of $W_1,W_2$. We denote the right-hand side of $(a)$ by $J^1_{t+1}(.)$ as in \eqref{eq: bound on linear drift of H^1 }. 
% Inequality $(b)$ follows because reducing conditioning increases the entropy.
Similarly for the case when $i=2$ the following lower-bound holds 
\begin{align}\nonumber
\EE[&H^2_{t+1}-H^2_{t}|m_1,y^t ]\\\nonumber
&= -H(Y_{t+1}|m_1, x_{1}^{t+1}, y^t )  +H(Y_{t+1}|X_{2}^{t+1}, x_{1}^{t+1},y^t)\\\label{eq: bound on linear drift of H^2 }
&\triangleq -J^2_{t+1}(m_1,x_{1}^{t+1},y^t).
\end{align}
Using a similar argument for the case when $i=3$, we can show that the following inequality holds 
\begin{align}\nonumber
\EE[H^3_{t+1}-H^3_{t}|y^t ]&\geq -I(X_{1}^{t+1},X_{2}^{t+1};Y_{t+1}| y^t)\\\label{eq: bound on linear drift of H^3 }
&\triangleq -J^3_{t+1}(y^t).
\end{align}
Consider the quantities at the right-hand side of \eqref{eq: bound on linear drift of H^1 }, \eqref{eq: bound on linear drift of H^2 } and \eqref{eq: bound on linear drift of H^3 }, i.e., the functions $J^1_{t+1}, J^2_{t+1},J^3_{t+1}$. We proceed by the following lemma. 

\begin{lem}
The vector $(J^1_{t+1}, J^2_{t+1},J^3_{t+1})$ is inside the feedback-capacity region $\mathcal{C}$ almost surely.
\end{lem}
\begin{IEEEproof}
We use the alternative representation for $\mathcal{C}$ which is given in Fact \ref{prop: MAC-FB capacity hyperplane}. For any non-negative numbers $\lambda_1, \lambda_2, \lambda_3$, let 
\begin{align*}
 J_{\lambda}(m_1,m_2,x_1^{t+1}, x_2^{t+1}, y^t)&=\lambda_1 J^1_{t+1}(m_2,x_{2}^{t+1},y^t)+\lambda_2 J^2_{t+1}(m_1,x_{1}^{t+1},y^t)+\lambda_3 J^3_{t+1}(y^t)
\end{align*}
 Note that 
\begin{align}\label{eq: bound on J lambda}
J_{\lambda}(m_1,& m_2, x_1^{t+1}, x_2^{t+1},y^t) \leq \sup_{P_{W_1W_2X^{t+1}_1X^{t+1}_2|Y^{t+1}}} \EE\{J_{\lambda}(W_1,W_2,X_1^{t+1}, X_2^{t+1}, y^t)\},
\end{align}
where the supremum is taken over all $P_{X^{t+1}_1X^{t+1}_2|Y^{t+1}}$ that factors as in \eqref{eq: factorization of P}.
The right-hand side of the above inequality  equals $\sum_i \EE[\lambda_i J^i_{t+1}]$. Each expectation inside the summation can be bounded as follows  
\begin{align*}
\EE\{J^1_{t+1}(W_2,X_{2}^{t+1},y^t)\}&=H(Y_{t+1}|W_2, X_{2}^{t+1}, y^t ) - H(Y_{t+1}|X_{2}^{t+1}, X_{1}^{t+1},y^t)\\
&\leq H(Y_{t+1}|X_{2}^{t+1}, y^t ) - H(Y_{t+1}|X_{2}^{t+1}, X_{1}^{t+1},y^t)\\
&=I(X_{1, t+1}, Y_{t+1}|X_{2}^{t+1}, y^t)
\end{align*}
Similarly, 
\begin{align*}
\EE\{J^2_{t+1}(W_1,X_{1}^{t+1},y^t)\}&\leq I(X_{2, t+1}; Y_{t+1}|X_1^{t+1}y^t)\\
\EE\{J^3_{t+1}(y^t)\}&\leq I(X_{1,t+1},X_{2,t+1};Y_{t+1}| y^t)
\end{align*}
Therefore, since the channel is memoryless using the above bounds we have
\begin{align*}
&\EE\{J_{\lambda}(W_1,W_2,X_1^{t+1}, X_2^{t+1}, y^t)\}\\
&\leq\lambda_1 I(X_{1, t+1}, Y_{t+1}|X_{2}^{t+1}, y^t) +\lambda_2 I(X_{2, t+1}; Y_{t+1}|X_1^{t+1}y^t)+\lambda_3 I(X_{1,t+1},X_{2,t+1};Y_{t+1}| y^t)\\
&\leq C_{\underline{\lambda}}
\end{align*}
\end{IEEEproof}
Since the vector $(J^1_{t+1}, J^2_{t+1},J^3_{t+1})$ is inside the capacity for all $1\leq t \leq N$, then, by definition, $\forall \epsilon>0$ there exist $L$ and $P_{X^{L}_1X^{L}_2 Y^{L}}$ factoring as in \eqref{eq: factorization of P} such that
 \begin{align*}
 J^i_{t+1} \leq I^i_L+\epsilon, \quad i=1,2,3
  \end{align*}
holds for all $1\leq t \leq N$. This implies the statement of the lemma.

\end{IEEEproof}
%
}








{
\section{Proof of Lemma \ref{lem: log drift MAC-FB} }\label{appx: proof of lem log drift}
\begin{IEEEproof}
We prove the first statement of the lemma. The second and the third statements follow by a similar argument. Given $Y^t=y^t, W_2=m$, define the following quantities
\begin{align*}
f_{i|m}&=P(W_1=i| Y^t=y^t, W_2=m)\\
f_{i|m}(y_{t+1})&=P(W_1=i| Y^t=y^t, W_2=m, Y_{t+1}=y_{t+1})\\
Q_{i,m}(y_{t+1})&=P(Y_{t+1}=y_{t+1}|W_1=i, W_2=m, Y^t=y^t),
\end{align*}
where $i\in [1:M_1], y_{t+1}\in \mathcal{Y}$.
Since $H^1_t < \epsilon$, then there exist $\epsilon'$ (as a function of $\epsilon$) and an index $l\in [1:M_1]$ such that $f_{l|m}\geq 1-\epsilon'$ and $f_{i|m}\leq \frac{\epsilon'}{M_1-1}$ for all $i\in [1:M_1], i\neq l$. Denote
\begin{align*}
\hat{f}_{i|m}=\frac{f_{i|m}}{1-f_{l|m}}, \quad  i\neq l.
\end{align*}
Using the grouping axiom we have
\begin{align*}
H^1_{t}=H(W_1|W_2=m, y^t)=h_b(f_{l|m})+(1-f_{l|m})H(\hat{X})
\end{align*}
where $\hat{X}$ is a random variable with probability distribution $P(\hat{X}=i)=\hat{f}_{i|m}, ~i\in [1:M_1], i\neq l$. Note that $$h_b(f_{l|m}) \approx -(1-f_{l|m})\log (1-f_{l|m}).$$ Therefore,
\begin{align}\nonumber
H^1_{t}&\approx -(1-f_{l|m})(\log(1-f_{l|m})-H(\hat{X}))\\\label{eq: approximate H^1_t}
&\approx (1-f_{l|m})\log(1-f_{l|m})
\end{align}
where the last approximation is due to the fact that $-\log(1-f_{l|m})\gg H(\hat{X})$. %   $-\log(1-f_{l|m})\geq -\log \epsilon' >> \log M_1 \geq H(\hat{X})$ 
 Next, we derive an approximation for $H^1_{t+1}$. Note that
\begin{align*}
f_{l|m}(y_{t+1})=\frac{f_{l|m}Q_{l,m}(y_{t+1})}{\sum_j f_{j|m}Q_{j,m}(y_{t+1})}
\end{align*}
The denominator can be written as 
$$f_{l|m}Q_{l,m}(y_{t+1})+(1-f_{l|m})\sum_{j\neq l} \hat{f}_{j|m}Q_{j,m}(y_{t+1}).$$
The above quantity is approximately equals to $Q_{l,m}(y)$. Therefore,
\begin{align*}
(1-f_{l|m}(y_{t+1}))&=(1-f_{l|m}) \frac{\sum_{j\neq l} \hat{f}_{j|m}Q_{j,m}(y_{t+1})}{\sum_j f_{j|m}Q_{j,m}(y_{t+1})}\\
&\approx (1-f_{l|m}) \frac{\sum_{j\neq l} \hat{f}_{j|m}Q_{j,m}(y_{t+1})}{Q_{l,m}(y_{t+1})}
\end{align*}
This implies that $f_{l|m}(y_{t+1}) \approx 1$. Therefore, using the same argument for $H^1_t$ we have
\begin{align}\nonumber
H^1_{t+1}&\approx -(1-f_{l|m}(y_{t+1}))(\log(1-f_{l|m}(y_{t+1}))\\\nonumber
&=-(1-f_{l|m}(y_{t+1}))\Big[\log(1-f_{l|m})+ \log (\frac{\sum_{j\neq l} \hat{f}_{j|m}Q_{j,m}(y_{t+1})}{Q_{l,m}(y_{t+1})})\Big]\\\label{eq: approximate H^1_t+1}
&\approx -(1-f_{l|m}(y_{t+1}))\log(1-f_{l|m}).
\end{align}
As a result of the approximations in \eqref{eq: approximate H^1_t} and \eqref{eq: approximate H^1_t+1}, we obtain
\begin{align*}
\frac{H^1_{t+1}}{H^1_{t}}&\approx \frac{(1-f_{l|m}(y))\log(1-f_{l|m})}{(1-f_{l|m})\log(1-f_{l|m})}\\
&=\frac{\sum_{j\neq l} \hat{f}_{j|m}Q_{j,m}(y)}{Q_{l,m}(y)}
\end{align*}
Note that
\begin{align*}
P(Y_{t+1}=y| W_2=m, y^t)\approx Q_{l,m}(y)
\end{align*}
Therefore, 
\begin{align*}
\EE\{\log \frac{H^1_{t+1}}{H^1_{t}}| y^t\}&\approx \EE\{\log \frac{\sum_{j\neq l} \hat{f}_{j|m}Q_{j,m}(Y_{t+1})}{Q_{l,m}(Y_{t+1})}\}\\
&=\sum_{y}Q_{l,m}(y) \log \frac{\sum_{j\neq l} \hat{f}_{j|m}Q_{j,m}(y)}{Q_{l,m}(y)}\\
&\stackrel{(a)}{=}-D(Q_{l,m}|| \sum_{j\neq l} \hat{f}_{j|m}Q_{j,m})\\
& \stackrel{(b)}{\geq}  -\sum_{j\neq l} \hat{f}_{j|m} D(Q_{l,m}|| Q_{j,m})\\
&\geq -\max_{j\neq l} D(Q_{l,m}|| Q_{j,m})\\
&\stackrel{(c)}{\geq}  -(D_1+\epsilon)
\end{align*}
where $(a)$ is due to the definition of Kullback–Leibler divergence, $(b)$ is due to the convexity of Kullback–Leibler divergence, and $(c)$ is due to the definition of $D_1$.
\end{IEEEproof}

}


%\section{proof of Lemma \ref{lem: Z_i are submartingale}}
%We need the following lemma to proceed. The lemma is a result of Lemma 4 in \cite{Burnashev}, and we omit its proof.
%\begin{lem}
%There exists a constant $K>0$ such that for any $t\geq 1$ and $i=1,2,3$, the following inequality holds almost surely w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2} \times \mathcal{F}_t$
%\begin{align*}
%\log H_t^i-\log H_{t+1}^i \leq K.
%\end{align*}
%\end{lem}
%We can show that the constant $K$ in the lemma is $$K=\max_{\substack{j,l\in [1:M_1]\\ k,m\in [1:M_2]}}\max_{y\in \mathcal{Y}} \frac{\hat{Q}_{j,k}(y)}{\hat{Q}_{l,m}(y)}.$$
%Suppose $W_2=m$ for some $m\in [1:M_2]$. Given this event and using the same argument as in the proof of Theorem 1 in \cite{Burnashev} we can show that $Z_{t}^{(i)}| W_2=m$ is a submartingale for all $m$. More precisely, the inequality
%\begin{align*}
%\EE\{Z_{t}^{(i)}-Z_{t+1}^{(i)}| \mathcal{F}_{W_1}\times \mathcal{F}_{W_2}\}\leq 0,
%\end{align*} 
%holds almost surely w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2}$. Taking the expectation of the both sides in the above inequality gives
%\begin{align*}
%\EE\{Z_{t}^{(i)}-Z_{t+1}^{(i)}\}\leq 0,\quad \forall t\geq 0, ~ i=1,2,3.
%\end{align*}
%Thus, $Z_{t}^{(i)}$ is a submartingale for $i=1,2,3$ and w.r.t $\mathcal{F}_{W_1}\times \mathcal{F}_{W_2}\times \mathcal{F}_t$.


==> proofs/proof_lem_logdrift_OLD.tex <==
\section{Proof of Lemma \ref{lem: log drift MAC FB} }\label{appx: proof of lem log drift}
\begin{IEEEproof}
We start with the case $i=1$. The proof for the other two cases follows from the same argument.  Define the following quantities
\begin{align*}
%f_{i|m}&=P(W_1=i| Y^t=y^t, W_2=m)\\
\mu_{1}(w)&=\prob{W_1=w| Y^{r-1}=y^{r-1}}\\
\mu_{1}(w, y_{r})&=\prob{W_1=w| Y^{r-1}=y^{r-1},Y_{r}=y_{r}}\\
Q^1_{w}(y_{r})&=\prob{Y_{r}=y_{r}|W_1=w, Y^{r-1}=y^{r-1}},
\end{align*}
where $i\in [1:M_1], y_{t+1}\in \mathcal{Y}$.

Let $w^*_{1,r} = \argmax_w \mu_1(w)$. First, we show that having $\Htld^1_{r-1} < \epsilon, \epsilon\in [0,\frac{1}{2}]$, we conclude that $\mu_1(\wstar)= 1-\epsilon'$, where $\epsilon'=o_1(\epsilon)$ with $o_1$ being a function satisfying $\lim_{\epsilon \rightarrow 0} o_1(\epsilon) =0.$ The argument is as follows:
%Using the grouping axiom we have
%\begin{align*}
%\Htld^1_{r-1}=H(W_1|y^{r-1})=h_b( \mu_1(w^*_{1,r}))+(1-\mu_1(w^*_{1,r}))H(\hat{W}_1) \geq h_b( \mu_1(w^*_{1,r}))+(1-\mu_1(w^*_{1,r}))
%\end{align*}
%where $\hat{W}_1$ is a random variable with probability distribution $P(\hat{W}_1=w)=\frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})}, ~w\in [1:M_1], w\neq w^*_{1,r}$. Hence, 
%\begin{align*}
% \epsilon \geq  h_b(\mu_1(\wstar)).
% \end{align*}



By grouping the messages $w\neq \wstar$ into a one combo message, we can write 
\begin{align*}
 \epsilon \geq \Htld^1_{r-1}\geq h_b(\mu_1(\wstar)).
 \end{align*} 
 Taking the inverse image of $h_b$ implies that $\mu_1(\wstar)\geq 1-h_b^{-1}(\epsilon)$ or $\mu_1(\wstar)\leq h_b^{-1}(\epsilon)$. The second inequality is not feasible because otherwise if $\epsilon=0$ then $\mu_1(\wstar)=0$ which is a contradiction as $\wstar$ is the MAP message. Hence, $\mu_1(\wstar)\geq 1-h_b^{-1}(\epsilon)$. Therefore, there exists a function $o_1(\epsilon)$ such that $\mu_1(\wstar)=1-o_1(\epsilon)$ and $0\leq o_1(\epsilon)\leq h_b^{-1}(\epsilon)$.



%there exist sufficiently small $\epsilon'\in (0,1)$ (as a function of $\epsilon$) such that $\mu_1(w^*_{1,r})= 1-\epsilon'$ and $\mu_1(w)\leq \frac{\epsilon'}{M_1-1}$ for all $w\neq w^*_{1,r}$. 
Next, using the grouping axiom we have that
\begin{align*}
\Htld^1_{r-1}=H(W_1|y^{r-1})=h_b( \mu_1(w^*_{1,r}))+(1-\mu_1(w^*_{1,r}))H(\hat{W}_1)
\end{align*}
where $\hat{W}_1$ is a random variable with probability distribution $P(\hat{W}_1=w)=\frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})}, ~w\in [1:M_1], w\neq w^*_{1,r}$. Note that $$h_b(\mu_1(w^*_{1,r})) \approx -(1-\mu_1(w^*_{1,r}))\log (1-\mu_1(w^*_{1,r})).$$ Therefore,
\begin{align}\nonumber
\Htld^1_{r-1}&\approx -(1-\mu_1(w^*_{1,r}))\big(\log(1-\mu_1(w^*_{1,r}))-H(\hat{W}_1)\big)\\\label{eq: approximate H^1_t}
&\approx (1-\mu_1(w^*_{1,r}))\log(1-\mu_1(w^*_{1,r}))
\end{align}
where the last approximation is due to the fact that $-\log(1-\mu_1(w^*_{1,r}))\gg H(\hat{W}_1)$. %   $-\log(1-f_{l|m})\geq -\log \epsilon' >> \log M_1 \geq H(\hat{X})$ 
 Next, we derive an approximation for $\Htld^1_{r}$. Note that
\begin{align*}
\mu_{1}(w^*_{1,r}, y_{r}) =\frac{\mu_1(w^*_{1,r})Q^1_{w^*_{1,r}}(y_{r})}{\sum_w \mu_1(w) Q_{w}^1(y_{r})}
\end{align*}
The denominator can be written as 
$$\mu_1(w^*_{1,r}) Q^1_{w^*_{1,r}}(y_{r})+(1-\mu_1(w^*_{1,r}))\sum_{w\neq w^*_{1,r}}  \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})}   Q^1_{w}(y_{r}).$$
The above quantity is approximately equals to $Q^1_{w^*_{1,r}}(y_{r})$. Therefore,
\begin{align}\nonumber
(1-\mu_{1}(w^*_{1,r}, y_{r}))&=(1-\mu_1(w^*_{1,r})) \frac{\sum_{w\neq w^*_{1,r}} \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})}   Q^1_{w}(y_{r})}{\sum_w \mu_1(w) Q_{w}^1(y_{r})}\\\label{eq:1-mu1 approximate}
&\approx (1-\mu_1(w^*_{1,r})) \frac{\sum_{w\neq w^*_{1,r}} \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})} Q^1_{w}(y_{r})}{Q^1_{w^*_{1,r}}(y_{r})}
\end{align}
This implies that $\mu_{1}(w^*_{1,r}, y_{r}) \approx 1$. Therefore, using the same argument for $\Htld^1_{r-1}$ we have that
\begin{align}\nonumber
\Htld^1_{r}&\approx -(1-\mu_{1}(w^*_{1,r}, y_{r}))(\log(1-\mu_{1}(w^*_{1,r}, y_{r}))\\\nonumber
&=-(1-\mu_{1}(w^*_{1,r}, y_{r}))\Bigg[\log(1-\mu_1(w^*_{1,r}))+ \log \Big(\frac{\sum_{w\neq w^*_{1,r}} \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})} Q^1_{w}(y_{r})}{Q^1_{w^*_{1,r}}(y_{r})}\Big)\Bigg]\\\label{eq: approximate H^1_t+1}
&\approx -(1-\mu_{1}(w^*_{1,r}, y_{r}))\log(1-\mu_1(w^*_{1,r})).
\end{align}
As a result of the approximations in \eqref{eq: approximate H^1_t} and \eqref{eq: approximate H^1_t+1}, we obtain that
\begin{align*}
\frac{\Htld^1_{r}}{\Htld^1_{r-1}}&\approx \frac{(1-\mu_{1}(w^*_{1,r}, y_{r}))\log(1-\mu_1(w^*_{1,r})}{(1-\mu_1(w^*_{1,r}))\log(1-\mu_1(w^*_{1,r}))}\\
&=\frac{\sum_{w\neq w^*_{1,r}} \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})} Q^1_{w}(y_{r})}{Q^1_{w^*_{1,r}}(y_{r})},
\end{align*}
where the last equality follows from \eqref{eq:1-mu1 approximate}. Note that
\begin{align*}
P(Y_{r}=y_r|Y^{r-1}=y^{r-1})\approx Q^1_{w^*_{1,r}}(y_{r}).
\end{align*}
Therefore, 
\begin{align*}
\EE_{Y_r}\{\log {\Htld^1_{r}}- \log {\Htld^1_{r-1}}| y^{r-1}\}&\approx \EE\Bigg\{\log \frac{\sum_{w\neq w^*_{1,r}} \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})} Q^1_{w}(Y_{r})}{Q^1_{w^*_{1,r}}(Y_{r})} \Big| y^{r-1}\Bigg\}\\\numberthis \label{eq:log drift bound 1}
&\approx \sum_{y_r}Q^1_{w^*_{1,r}}(y_{r}) \log \frac{\sum_{w\neq w^*_{1,r}} \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})} Q^1_{w}(y_{r})}{Q^1_{w^*_{1,r}}(y_{r})}
%&=-D_{KL}\Big(Q^1_{w^*_{1,r}}(\cdot)|| \sum_{w\neq w^*_{1,r}} \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})} Q^1_{w}(\cdot)\Big)\\
%&= -\D^1_r,
%& \stackrel{(b)}{\geq}  -\sum_{j\neq l} \hat{f}_{j|m} D(Q_{l,m}|| Q_{j,m})\\
%&\geq -\max_{j\neq l} D(Q_{l,m}|| Q_{j,m})\\
%&\stackrel{(c)}{\geq}  -(D_1+\epsilon)
\end{align*}
Note that the right-hand side of \eqref{eq:log drift bound 1} depends on the messages. In what follows we remove this dependency. Let $\Qbar = P_{Y_r|X_{1,r}, Y^{r-1}}$ which is the effective channel from the first user's perspective at time $r$. Let $\nu_1(x) = \PP\{X_1=x | Y^{r-1}=y^{r-1}\}$ and define 
\begin{align*}
\xstar = \argmax_{x_1 \in \mathcal{X}_1} \nu_1(x_1).
\end{align*}
We show that 
\begin{align*}
 \eqref{eq:log drift bound 1} \geq -D_{KL}\Big(\Qbar(\cdot | \xstar, y^{r-1})|| \sum_{x_1\neq \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar(\cdot| x_1, y^{r-1})\Big)
 \end{align*} 
 Repeating the above argument for $i=2,3$ completes the proof of the lemma. Hence, it remains to prove the above inequality. 

We proceed by bounding  $Q^1_{\wstar}(y_{r})$. Since $X_{1,r}=e_1(W_1, Y^{r-1}),$ then $\xstar = e_1(\wstar, y^{r-1}).$ Hence, we have that 
\begin{align*}
Q^1_{\wstar}(y_{r}) &= \prob{Y_r = y_r \big|~ W_1 = \wstar, Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
&= \sum_{x_2 \in\mathcal{X}_2} \prob{Y_r = y_r, X_{2,r} = x_2 \big|~ W_1 = \wstar, Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\\numberthis \label{eq:Q1 Qbar eq 1}
&= \sum_{x_2 \in\mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~ W_1 = \wstar, Y^{r-1}=y^{r-1}, X_{1,r} = \xstar }Q(y_r| x_2, \xstar)
%&= \sum_{x_2 \in\mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} = \xstar }\frac{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar, X_{2,r} = x_2\}}{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar\}}Q(y_r| x_2, \xstar),
\end{align*}
where the last equality holds as the channel is memoryless.  Next, we bound the conditional probability on $X_{2,r}$ in the above summation. This quantity equals to 
 \begin{align*}
\prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} = \xstar }\frac{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar, X_{2,r} = x_2\}}{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar\}}
 \end{align*}
 The denominator is greater than $(1-\epsilon')$ because of the following argument: 
 \begin{align*}
\prob{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} &= \frac{\PP\{W_1= \wstar, X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}{\PP\{X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}\\
 &= \frac{\PP\{W_1= \wstar| Y^{r-1}=y^{r-1}\}}{\PP\{X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}\\
 &\geq \frac{1-\epsilon'}{\PP\{X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}\\
 &\geq 1-\epsilon'.
 \end{align*}
As the nominator is less than one, then from  \eqref{eq:Q1 Qbar eq 1}, we have that 
  \begin{align*}
Q^1_{\wstar}(y_{r}) & \leq \frac{1}{1-\epsilon'}\sum_{x_2 \in\mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} = \xstar } Q(y_r| x_2, \xstar)\\\numberthis \label{eq:Q1 Qbar bound 1}
& = \frac{1}{1-\epsilon'} \Qbar(y_r| \xstar, y^{r-1}).
 \end{align*}
 Next, we bound the next term that appeared in \eqref{eq:log drift bound 1} as in the following
 \begin{align*}
\sum_{w\neq w^*_{1,r}}& \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})} Q^1_{w}(y_r) =  \frac{1}{1-\mu_1(w^*_{1,r})}\sum_{w\neq w^*_{1,r}} \prob{W_1= w, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& \stackrel{(a)}{\geq} \frac{1}{1-\mu_1(w^*_{1,r})}\sum_{\substack{w\neq \wstar,\\ x_1\neq \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{W_1= w, X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& \stackrel{(b)}{\geq} \frac{1}{1-\mu_1(w^*_{1,r})}\sum_{\substack{w\\ x_1\neq \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{W_1= w, X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& =\frac{1}{1-\mu_1(w^*_{1,r})}\sum_{\substack{x_1\neq \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& = \frac{1}{1-\mu_1(w^*_{1,r})}\sum_{\substack{x_1\neq \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{X_{1,r} = x_1, X_{2,r} = x_2\big|~Y^{r-1}= y^{r-1} }Q(y_r | x_1,x_2)\\
& \stackrel{(c)}{=} \frac{1}{1-\mu_1(w^*_{1,r})}\sum_{\substack{x_1\neq \xstar}} \prob{X_{1,r} = x_1 \big|~Y^{r-1}= y^{r-1} } \sum_{x_2\in\mathcal{X}_2} \prob{X_{2,r} = x_2\big|~Y^{r-1}= y^{r-1},X_{1,r} = x_1 } Q(y_r | x_1,x_2)\\
&\stackrel{(d)}{=} \frac{1}{1-\mu_1(w^*_{1,r})}\sum_{\substack{x_1\neq \xstar}} \nu_1(x_1) \Qbar(y_r|x_1, y^{r-1})\\\numberthis \label{eq:Q1 Qbar bound 2}
& \stackrel{(e)}{\approx} \frac{1}{1-\nu_1(\xstar)}\sum_{\substack{x_1\neq \xstar}} \nu_1(x_1) \Qbar(y_r|x_1, y^{r-1}),
 \end{align*}
 where (a) holds by summing over $x_1$ and $x_2$. Note that this is an inequality because the summation is not over all values of $x_1$. Equality (b) holds by removing the condition $w\neq \wstar$. This is an equality, because the probability of the event $\{W_1 =\wstar, X_{1,r} \neq \xstar\}$ is zero. Equality (c) follows by breaking the joint probability on $(X_{1,r}, X_{2,r})$ and further moving the summation on $x_2$. Equality (d) is due to the definition of $\nu_1$ and $\Qbar$. Lastly, (e) is due to the fact that $\nu_1(\xstar) \approx \mu_1(\wstar) = 1-\epsilon'$. 
 
With the bounds in \eqref{eq:Q1 Qbar bound 1} and \eqref{eq:Q1 Qbar bound 2}, the log-drift in \eqref{eq:log drift bound 1} is bounded as 
 \begin{align*}
 \EE_{Y_r}\{\log {\Htld^1_{r}}- \log {\Htld^1_{r-1}}| y^{r-1}\}&\approx \sum_{y_r}Q^1_{w^*_{1,r}}(y_{r}) \log \frac{\sum_{w\neq w^*_{1,r}} \frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})} Q^1_{w}(y_{r})}{Q^1_{w^*_{1,r}}(y_{r})}\\
&\stackrel{(a)}{\geq}  \sum_{y_r}Q^1_{w^*_{1,r}}(y_{r}) \log \frac{\sum_{x_1\neq \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar(y_{r}|x_1, y^{r-1})}{\frac{1}{1-\epsilon'}\Qbar(y_{r}|\xstar, y^{r-1})}\\
&\stackrel{(b)}{\approx} \sum_{y_r}\Qbar(y_{r}|\xstar, y^{r-1}) \log \frac{\sum_{x_1\neq \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar(y_{r}|x_1, y^{r-1})}{\frac{1}{1-\epsilon'}\Qbar(y_{r}|\xstar, y^{r-1})}\\
& = -D_{KL}\Big(\Qbar(\cdot | \xstar, y^{r-1})|| \sum_{x_1\neq \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar(\cdot| x_1, y^{r-1})\Big)+\log (1-\epsilon'),
 \end{align*}
 where (a) follows from \eqref{eq:Q1 Qbar bound 1} and \eqref{eq:Q1 Qbar bound 2}, and (b) follows from the following argument: 
\begin{align*}
Q^1_{\wstar}(y_{r}) &= \prob{Y_r = y_r \big|~ W_1 = \wstar, Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%&= \frac{\prob{Y_r = y_r, W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}}{\prob{W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}}\\
& \geq \prob{Y_r = y_r, W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
& = \prob{Y_r = y_r \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} \prob{ W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar, Y_r = y_r}\\
&=\Qbar(y_r|\xstar, y^{r-1}) \frac{\prob{ W_1 = \wstar, X_{1,r} = \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}{\prob{X_{1,r} = \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}\\
&\stackrel{(a)}{=}\Qbar(y_r|\xstar, y^{r-1}) \frac{\prob{ W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}{\prob{X_{1,r} = \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}\\
&\stackrel{(b)}{=} \Qbar(y_r|\xstar, y^{r-1})\prob{ W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}\\
& \stackrel{(c)}{=} \Qbar(y_r|\xstar, y^{r-1}) \mu_1(\wstar, y_r),\\
& \stackrel{(d)}{\approx} \Qbar(y_r|\xstar, y^{r-1})
%
%& = \sum_{w}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} - \sum_{w\neq \wstar}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%& = \prob{Y_r = y_r \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} - \sum_{w\neq \wstar}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%& = \Qbar(y_r|\xstar, y^{r-1}) - \prob{Y_r = y_r, W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%& \geq \Qbar(y_r|\xstar, y^{r-1}) - \prob{W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
 \end{align*} 
where  (a) holds as $X_{1,r}$ is a function of $(W_1, Y^{r-1}$, (b) holds as the denominator is less than one, (c) is due to the definition of $\mu_1(w_1, y_r)$, and (d) holds as $\mu_1(\wstar, y_r)\approx 1$ as discussed in \eqref{eq:1-mu1 approximate}.
 
%\begin{align*}
%\prob{Y_r = y_r, W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} & = \frac{\prob{Y_r = y_r, W_1 \neq \wstar, X_{1,r} = \xstar \big|~ Y^{r-1}=y^{r-1}}}{\prob{X_{1,r} = \xstar \big|~ Y^{r-1}=y^{r-1}}}\\
%& \leq \frac{\prob{W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}}}{\nu_1(\xstar)}\\
%& \leq \frac{\epsilon'}{\nu_1(\xstar)}\\
%&\leq \frac{\epsilon'}{1-\epsilon'}
% \end{align*} 
 
\end{IEEEproof}


==> proofs/proof_lem_logdrift_v1.tex <==
\section{Proof of Lemma \ref{lem: log drift MAC FB} }\label{appx: proof of lem log drift}
\begin{IEEEproof}
We start with the case $i=1$. The proof for the other two cases follows from the same argument.  Define the following quantities
\begin{align*}
%f_{i|m}&=P(W_1=i| Y^t=y^t, W_2=m)\\
\mu_{1}(w)&=\prob{W_1=w| Y^{r-1}=y^{r-1}}\\
\mu_{1}(w, y_{r})&=\prob{W_1=w| Y^{r-1}=y^{r-1},Y_{r}=y_{r}}\\
Q^1_{w}(y_{r})&=\prob{Y_{r}=y_{r}|W_1=w, Y^{r-1}=y^{r-1}},
\end{align*}
where $i\in [1:M_1], y_{t+1}\in \mathcal{Y}$. 
 
Let $\Wstar \in [1: M_1]$ be the most likely message condition on $y^{r-1}$. That is $\wstar = \max_{w\in [1: M_1]}\mu_{1}(w)$.
First, we show that having $\Htld^1_{r-1} < \epsilon, \epsilon\in [0,1)$, we conclude that $\mu_1(\wstar)= 1-\eta_1(\epsilon)$ with $\eta_1$ being a function satisfying $\lim_{\epsilon \rightarrow 0} \eta_1(\epsilon) =0.$ The argument is as follows:
 
Using the grouping axiom we have
\begin{align}\label{eq:Htld eq 1}
\Htld^1_{r-1}=H(W_1|y^{r-1})=h_b( \mu_1(w^*_{1,r}))+(1-\mu_1(w^*_{1,r}))H(\hat{W}_1), 
%\geq h_b( \mu_1(w^*_{1,r}))+(1-\mu_1(w^*_{1,r}))
\end{align}
where $\hat{W}_1$ is a random variable with probability distribution $P(\hat{W}_1=w)=\frac{\mu_1(w)}{1-\mu_1(w^*_{1,r})}, ~w\in [1:M_1], w\neq w^*_{1,r}$. Hence, having $\Htld^1_{r-1}\leq \epsilon$ implies that $h_b(\mu_1(\wstar))\leq \epsilon$.
Taking the inverse image of $h_b$ implies that either $\mu_1(\wstar)\geq 1-h_b^{-1}(\epsilon)$ or $\mu_1(\wstar)\leq h_b^{-1}(\epsilon)$, where $h_b^{-1}:[0,1]\rightarrow [0,\frac{1}{2}]$ is the lower-half inverse function of $h_b$.  We show that the second  case is not feasible. For this purpose, we show that the inequality $\mu_1(\wstar)\leq h_b^{-1}(\epsilon)\leq \frac{1}{2}$ implies that $\Htld^1_{r-1}\geq 1$ which is a contradiction  with the original assumption $\Htld^1_{r-1} \leq \epsilon < 1$. This statement is proved in the following proposition. With this argument, we conclude that $\Htld^1_{r-1}\leq \epsilon$ implies that $\mu_1(\wstar)\geq 1-\eta_1(\epsilon)$, where $\eta_1(\cdot) = h_b^{-1}(\cdot)$.

\begin{proposition}
Let $W$ be a random variable taking values from a finite set $\mathcal{W}$. Suppose that $P_W(w)\leq \frac{1}{2}$ for all $w\in \mathcal{W}$. Then $H(W)\geq 1$. 
\end{proposition}
\begin{proof}
The proof follows from an induction on $|\mathcal{W}|$. For $|\mathcal{W}|=2$ the condition in the statement implies that $W$ has uniform distribution and hence $H(W)=1$ trivially. Suppose the statement holds for $|\mathcal{W}|=n-1$. Then, we prove it for $|\mathcal{W}|=n$.  Sort elements of $\mathcal{W}$ in an descending order according to $P_W(w)$, from the most likely (denoted by $w_1$) to the least likely ($w_n$). If $P_W(w_n)=0$, then the statement holds trivially from the induction's hypothesis.  Suppose $P_W(w_n)>0$. In this case, we can reduce  $H(W)$ by increasing $P_W(w_1)$ and decreasing $P_W(w_n)$ so that $P_W(w_1)+P_W(w_n)$ remains constant. In that case, either $P_W(w_n)$ becomes zero or $P_W(w_1)$ reaches the limit $\frac{1}{2}$. The first case happens if $P_W(w_1)+P_W(w_n)\leq \frac{1}{2}$. For that, the statement $H(W)\geq 1$ follows from the induction's hypothesis, as there are only $(n-1)$ elements with non-zero probability.  It remains to consider the second case in which $P_W(w_1)=\frac{1}{2}$ and $P_W(w_n)>0$. Again, we can further reduce the entropy by increasing $P_W(w_2)$ and decreasing $P_W(w_n)$ while $P_W(w_2)+P_W(w_n)$ remains constant. Observe that $P_W(w_2)+P_W(w_n)\leq \frac{1}{2}$ as $\sum_{i=2}^n P_W(w_i) = 1-P_W(w_1)=\frac{1}{2}$ and $p_W(w_i)>0$.  Hence, after this redistribution process $P_W(w_n)$ becomes zero. Then, the statement $H(W)\geq 1$ follows from the induction's hypothesis, as there are only $(n-1)$ elements with non-zero probability.
\end{proof}

%By grouping the messages $w\neq \wstar$ into a one combo message, we can write 
%\begin{align*}
% \epsilon \geq \Htld^1_{r-1}\geq h_b(\mu_1(\wstar)).
% \end{align*} 
% Taking the inverse image of $h_b$ implies that $\mu_1(\wstar)\geq 1-h_b^{-1}(\epsilon)$ or $\mu_1(\wstar)\leq h_b^{-1}(\epsilon)$. The second inequality is not feasible because otherwise if $\epsilon=0$ then $\mu_1(\wstar)=0$ which is a contradiction as $\wstar$ is the MAP message. Hence, $\mu_1(\wstar)\geq 1-h_b^{-1}(\epsilon)$. Therefore, there exists a function $o_1(\epsilon)$ such that $\mu_1(\wstar)=1-o_1(\epsilon)$ and $0\leq o_1(\epsilon)\leq h_b^{-1}(\epsilon)$.



%there exist sufficiently small $\epsilon'\in (0,1)$ (as a function of $\epsilon$) such that $\mu_1(w^*_{1,r})= 1-\epsilon'$ and $\mu_1(w)\leq \frac{\epsilon'}{M_1-1}$ for all $w\neq w^*_{1,r}$. 
We proceed with the proof of the lemma by approximating the right hand-side of \eqref{eq:Htld eq 1}. With $\mu_1(\Wstar)\geq 1-\eta_1(\epsilon)$, we have that 
\begin{align*}
h_b(\mu_1(\Wstar)) &=-\mu_1(\Wstar) \log \mu_1(\Wstar) - (1-\mu_1(\Wstar))\log (1-\mu_1(\Wstar))\\
& = - (1-\mu_1(\Wstar))\log (1-\mu_1(\Wstar))+\eta_2(\epsilon) 
\end{align*}
where the second equality is due to the Taylor's theorem for expanding $x\log x$ around $x=1$; with that, $x\log x = (x-1) + \zeta (x-1)^2$ for some $\zeta$ between $x$ and $1$. Hence, the second equality above holds as $x= \mu_1(\Wstar)\geq 1-\eta_1(\epsilon)$ and $\eta_2(\epsilon) =\eta_1(\epsilon)-\zeta \eta_1(\epsilon)^2$.  
 Therefore,
\begin{align}\nonumber
\Htld^1_{r-1}&=-(1-\mu_1(\Wstar))\big(\log(1-\mu_1(\Wstar))-H(\hat{W}_1)\big)+\eta_2(\epsilon) \\\label{eq: approximate H^1_t}
&\leq -(1-\mu_1(\Wstar))\log(1-\mu_1(\Wstar) + \eta_1(\epsilon) \log M_1+\eta_2(\epsilon).
\end{align}
On the other hand
\begin{align*}
\Htld^1_{r-1} \geq -(1-\mu_1(\Wstar))\log(1-\mu_1(\Wstar)+\eta_2(\epsilon)
\end{align*}
Therefore, if $\eta_1(\epsilon) \log M_1<<1 $, then $\Htld^1_{r-1}\approx -(1-\mu_1(\Wstar))\log(1-\mu_1(\Wstar)$.
 %   $-\log(1-f_{l|m})\geq -\log \epsilon' >> \log M_1 \geq H(\hat{X})$ 
 Next, we derive an approximation for $\Htld^1_{r}$. Suppose $y_r\in \mathcal{Y}$ has probability greater than 
\begin{align*}
 \prob{Y_r=y_r ~|~ y^{r-1}} = \sum_w \mu_1(w) Q_{w}^1(y_{r}) \geq  \sqrt{\eta_1(\epsilon)}
 \end{align*} 
 
  Note that
\begin{align*}
\mu_{1}(\Wstar, y_{r}) =\frac{\mu_1(\Wstar)Q^1_{\Wstar}(y_{r})}{\sum_w \mu_1(w) Q_{w}^1(y_{r})}
\end{align*}
%The denominator can be written as 
%$$\mu_1(\Wstar) Q^1_{\Wstar}(y_{r})+(1-\mu_1(\Wstar))\sum_{w\notin \Wstar}  \frac{\mu_1(w)}{1-\mu_1(\Wstar)}   Q^1_{w}(y_{r}) =  Q^1_{\Wstar}(y_{r})+ o_2(\epsilon),$$
%where  $o_2(\epsilon)\leq 2\epsilon$ is the residual term above.
 Therefore,
\begin{align}\label{eq:1-mu1 approximate}
(1-\mu_{1}(\Wstar, y_{r}))&=(1-\mu_1(\Wstar)) \frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)}   Q^1_{w}(y_{r})}{\sum_w \mu_1(w) Q_{w}^1(y_{r})}= \eta_3(\epsilon),
\end{align}
where $\eta_3(\epsilon) \leq \sqrt{\eta_1(\epsilon)}.$ Hence, having $\epsilon << 1$
implies that $\mu_{1}(\Wstar, y_{r}) \approx 1$. We use the same argument as for $\Htld^1_{r-1}$ to approximate $\Htld^1_r$. Therefore, from the right-hand side of \eqref{eq: approximate H^1_t} with $\epsilon$ replaced by $\eta_3(\epsilon)$, we have that
\begin{align}\nonumber
\Htld^1_{r}& \leq  -(1-\mu_{1}(\Wstar, y_{r}))(\log(1-\mu_{1}(\Wstar, y_{r}))+ \eta_3(\epsilon)\log M_1+
\eta_2(\eta_3(\epsilon))\\\nonumber
&=-(1-\mu_{1}(\Wstar, y_{r}))\Bigg[\log(1-\mu_1(\Wstar))+ \log \Big(\frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(y_{r})}{\sum_w \mu_1(w) Q_{w}^1(y_{r})}\Big)\Bigg]+ \eta_3(\epsilon)\log M_1+
\eta_2(\eta_3(\epsilon))\\\label{eq: approximate H^1_t+1}
&\leq  -(1-\mu_{1}(\Wstar, y_{r}))\log(1-\mu_1(\Wstar))+\eta_3(\epsilon) \log \Big(\frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(y_{r})}{\sum_w \mu_1(w) Q_{w}^1(y_{r})}\Big)+ \eta_3(\epsilon)\log M_1+
\eta_2(\eta_3(\epsilon)),
\end{align}
where $o_4(\epsilon) \leq  |\epsilon \log \epsilon|$.
As a result of the approximations in \eqref{eq: approximate H^1_t} and \eqref{eq: approximate H^1_t+1}, we obtain that
\begin{align*}
\frac{\Htld^1_{r}}{\Htld^1_{r-1}}&\approx \frac{(1-\mu_{1}(\Wstar, y_{r}))\log(1-\mu_1(\Wstar))}{(1-\mu_1(\Wstar))\log(1-\mu_1(\Wstar))}\\
&=\frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(y_{r})}{Q^1_{\Wstar}(y_{r})},
\end{align*}
where the last equality follows from \eqref{eq:1-mu1 approximate}. Note that
\begin{align*}
P(Y_{r}=y_r|Y^{r-1}=y^{r-1})\approx Q^1_{\Wstar}(y_{r}).
\end{align*}
Therefore, 
\begin{align*}
\EE_{Y_r}\{\log {\Htld^1_{r}}- \log {\Htld^1_{r-1}}| y^{r-1}\}&\approx \EE\Bigg\{\log \frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(Y_{r})}{Q^1_{\Wstar}(Y_{r})} \Big| y^{r-1}\Bigg\}\\\numberthis \label{eq:log drift bound 1}
&\approx \sum_{y_r}Q^1_{\Wstar}(y_{r}) \log \frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(y_{r})}{Q^1_{\Wstar}(y_{r})}
\end{align*}
Note that the right-hand side of \eqref{eq:log drift bound 1} depends on the messages. In what follows we remove this dependency. Let $\Qbar = P_{Y_r|X_{1,r}, Y^{r-1}}$ which is the effective channel from the first user's perspective at time $r$. Let $\nu_1(x) = \PP\{X_1=x | Y^{r-1}=y^{r-1}\}$ and define 
\begin{align*}
\Xstar  = e_1(\Wstar, y^{r-1})
%\xstar = \argmax_{x_1 \in \mathcal{X}_1} \nu_1(x_1).
\end{align*}
We show that 
\begin{align*}
 \eqref{eq:log drift bound 1} \geq -D_{KL}\Big(\Qbar(\cdot | \xstar, y^{r-1})|| \sum_{x_1\neq \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar(\cdot| x_1, y^{r-1})\Big)
 \end{align*} 
 Repeating the above argument for $i=2,3$ completes the proof of the lemma. Hence, it remains to prove the above inequality. 

We proceed by bounding  $Q^1_{\wstar}(y_{r})$. Since $X_{1,r}=e_1(W_1, Y^{r-1}),$  we have that 
\begin{align*}
Q^1_{\wstar}(y_{r}) &= \prob{Y_r = y_r \big|~ W_1 \in  \wstar, Y^{r-1}=y^{r-1}, X_{1,r} \in  \xstar}\\
&= \sum_{x_2 \in\mathcal{X}_2} \prob{Y_r = y_r, X_{2,r} = x_2 \big|~ W_1 \in \wstar, Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar}\\\numberthis \label{eq:Q1 Qbar eq 1}
&= \sum_{x_2 \in\mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~ W_1 \in \wstar, Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar }Q(y_r| x_2, \xstar)
%&= \sum_{x_2 \in\mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} = \xstar }\frac{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar, X_{2,r} = x_2\}}{\PP\{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar\}}Q(y_r| x_2, \xstar),
\end{align*}
where the last equality holds as the channel is memoryless.  Next, we bound the conditional probability on $X_{2,r}$ in the above summation. This quantity equals to 
 \begin{align*}
\prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar }\frac{\PP\{W_1\in \wstar | Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar, X_{2,r} = x_2\}}{\PP\{W_1\in \wstar | Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar\}}
 \end{align*}
 The denominator is greater than $(1-\epsilon')$ because of the following argument: 
 \begin{align*}
\prob{W_1= \wstar | Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} &= \frac{\PP\{W_1= \wstar, X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}{\PP\{X_{1,r} = \xstar | Y^{r-1}=y^{r-1}\}}\\
 &= \frac{\PP\{W_1\in \wstar| Y^{r-1}=y^{r-1}\}}{\PP\{X_{1,r} \in \xstar | Y^{r-1}=y^{r-1}\}}\\
 &\geq \frac{1-\epsilon'}{\PP\{X_{1,r} \in \xstar | Y^{r-1}=y^{r-1}\}}\\
 &\geq 1-\epsilon'.
 \end{align*}
As the nominator is less than one, then from  \eqref{eq:Q1 Qbar eq 1}, we have that 
  \begin{align*}
Q^1_{\wstar}(y_{r}) & \leq \frac{1}{1-\epsilon'}\sum_{x_2 \in\mathcal{X}_2} \prob{X_{2,r} = x_2 \big|~  Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar } Q(y_r| x_2, \xstar)\\\numberthis \label{eq:Q1 Qbar bound 1}
& = \frac{1}{1-\epsilon'} \Qbar(y_r| \xstar, y^{r-1}).
 \end{align*}
 Next, we bound the next term that appeared in \eqref{eq:log drift bound 1} as in the following
 \begin{align*}
\sum_{w \notin \Wstar }& \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(y_r) =  \frac{1}{1-\mu_1(\Wstar)}\sum_{w \notin \Wstar} \prob{W_1= w, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& \stackrel{(a)}{\geq} \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{w \notin  \wstar,\\ x_1\notin  \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{W_1= w, X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& \stackrel{(b)}{=} \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{w\\ x_1 \notin \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{W_1= w, X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& =\frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{x_1 \notin  \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{X_{1,r} = x_1, X_{2,r} = x_2, Y_r = y_r \big|~Y^{r-1}= y^{r-1} }\\
& = \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{x_1\notin \xstar}} \sum_{x_2\in\mathcal{X}_2} \prob{X_{1,r} = x_1, X_{2,r} = x_2\big|~Y^{r-1}= y^{r-1} }Q(y_r | x_1,x_2)\\
& \stackrel{(c)}{=} \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{x_1\notin  \xstar}} \prob{X_{1,r} = x_1 \big|~Y^{r-1}= y^{r-1} } \sum_{x_2\in\mathcal{X}_2} \prob{X_{2,r} = x_2\big|~Y^{r-1}= y^{r-1},X_{1,r} = x_1 } Q(y_r | x_1,x_2)\\
&\stackrel{(d)}{=} \frac{1}{1-\mu_1(\Wstar)}\sum_{\substack{x_1\notin  \xstar}} \nu_1(x_1) \Qbar(y_r|x_1, y^{r-1})\\\numberthis \label{eq:Q1 Qbar bound 2}
& \stackrel{(e)}{\approx} \frac{1}{1-\nu_1(\xstar)}\sum_{\substack{x_1\notin  \xstar}} \nu_1(x_1) \Qbar(y_r|x_1, y^{r-1}),
 \end{align*}
 where (a) holds by summing over $x_1$ and $x_2$. Note that this is an inequality because the summation is not over all values of $x_1$. Equality (b) holds by removing the condition $w\neq \wstar$. This is an equality, because the probability of the event $\{W_1 =\wstar, X_{1,r} \neq \xstar\}$ is zero. Equality (c) follows by breaking the joint probability on $(X_{1,r}, X_{2,r})$ and further moving the summation on $x_2$. Equality (d) is due to the definition of $\nu_1$ and $\Qbar$. Lastly, (e) is due to the fact that $\nu_1(\xstar) \approx \mu_1(\wstar) = 1-\epsilon'$. 
 
With the bounds in \eqref{eq:Q1 Qbar bound 1} and \eqref{eq:Q1 Qbar bound 2}, the log-drift in \eqref{eq:log drift bound 1} is bounded as 
 \begin{align*}
 \EE_{Y_r}\{\log {\Htld^1_{r}}- \log {\Htld^1_{r-1}}| y^{r-1}\}&\approx \sum_{y_r}Q^1_{\Wstar}(y_{r}) \log \frac{\sum_{w\notin \Wstar} \frac{\mu_1(w)}{1-\mu_1(\Wstar)} Q^1_{w}(y_{r})}{Q^1_{\Wstar}(y_{r})}\\
&\stackrel{(a)}{\geq}  \sum_{y_r}Q^1_{\Wstar}(y_{r}) \log \frac{\sum_{x_1\notin \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar(y_{r}|x_1, y^{r-1})}{\frac{1}{1-\epsilon'}\Qbar(y_{r}|\xstar, y^{r-1})}\\
&\stackrel{(b)}{\approx} \sum_{y_r}\Qbar(y_{r}|\xstar, y^{r-1}) \log \frac{\sum_{x_1\notin \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar(y_{r}|x_1, y^{r-1})}{\frac{1}{1-\epsilon'}\Qbar(y_{r}|\xstar, y^{r-1})}\\
& = -D_{KL}\Big(\Qbar(\cdot | \xstar, y^{r-1})|| \sum_{x_1\neq \xstar} \frac{\nu_1(x_1)}{1-\nu_1(\xstar)} \Qbar(\cdot| x_1, y^{r-1})\Big)+\log (1-\epsilon'),
 \end{align*}
 where (a) follows from \eqref{eq:Q1 Qbar bound 1} and \eqref{eq:Q1 Qbar bound 2}, and (b) follows from the following argument: 
\begin{align*}
Q^1_{\wstar}(y_{r}) &= \prob{Y_r = y_r \big|~ W_1 \in \wstar, Y^{r-1}=y^{r-1}, X_{1,r}\in \xstar}\\
%&= \frac{\prob{Y_r = y_r, W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}}{\prob{W_1 = \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar}}\\
& \geq \prob{Y_r = y_r, W_1 \in \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar}\\
& = \prob{Y_r = y_r \big|~ Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar} \prob{ W_1 \in \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} \in \xstar, Y_r = y_r}\\
&=\Qbar(y_r|\xstar, y^{r-1}) \frac{\prob{ W_1 \in \wstar, X_{1,r} \in \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}{\prob{X_{1,r} \in \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}\\
&\stackrel{(a)}{=}\Qbar(y_r|\xstar, y^{r-1}) \frac{\prob{ W_1 \in \wstar \big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}{\prob{X_{1,r}\in \xstar,\big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}}\\
&\stackrel{(b)}{=} \Qbar(y_r|\xstar, y^{r-1})\prob{ W_1 \in \wstar \big|~ Y^{r-1}=y^{r-1}, Y_r = y_r}\\
& \stackrel{(c)}{=} \Qbar(y_r|\xstar, y^{r-1}) \mu_1(\wstar, y_r),\\\numberthis\label{eq:Q1 Qbar bound 2}
& \stackrel{(d)}{\approx} \Qbar(y_r|\xstar, y^{r-1})
%
%& = \sum_{w}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} - \sum_{w\neq \wstar}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%& = \prob{Y_r = y_r \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} - \sum_{w\neq \wstar}\prob{Y_r = y_r, W_1 = w\big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%& = \Qbar(y_r|\xstar, y^{r-1}) - \prob{Y_r = y_r, W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
%& \geq \Qbar(y_r|\xstar, y^{r-1}) - \prob{W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar}\\
 \end{align*} 
where  (a) holds as $X_{1,r}$ is a function of $(W_1, Y^{r-1})$, (b) holds as the denominator is less than one, (c) is due to the definition of $\mu_1(w_1, y_r)$, and (d) holds as $\mu_1(\wstar, y_r)\approx 1$ as discussed in \eqref{eq:1-mu1 approximate}.
 
%\begin{align*}
%\prob{Y_r = y_r, W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}, X_{1,r} = \xstar} & = \frac{\prob{Y_r = y_r, W_1 \neq \wstar, X_{1,r} = \xstar \big|~ Y^{r-1}=y^{r-1}}}{\prob{X_{1,r} = \xstar \big|~ Y^{r-1}=y^{r-1}}}\\
%& \leq \frac{\prob{W_1 \neq \wstar \big|~ Y^{r-1}=y^{r-1}}}{\nu_1(\xstar)}\\
%& \leq \frac{\epsilon'}{\nu_1(\xstar)}\\
%&\leq \frac{\epsilon'}{1-\epsilon'}
% \end{align*} 
 
\end{IEEEproof}


==> proofs/thm_proof_lowerbound.tex <==
\section{Proof of Theorem \ref{thm: Error Exp lowerbound} }\label{appx: proof of thm error Exp lowebound}
\begin{IEEEproof}
{
At each block a re-transmission occurs  with probability $q$, an error occurs with probability $P_{eb}$ and a correct decoding process happens with probability $1-q-P_{eb}$. Let $\hat{\mathcal{H}}$ denote the decoders declared hypothesis. The probability of a re-transmission at each block is 
\begin{align*}
q=P(\hat{\mathcal{H}} = \mathcal{H}_1).
\end{align*}
The probability of error at each block is
\begin{align*}
P_{eb}=P(\mathcal{H}_1)P(\hat{\mathcal{H}} = \mathcal{H}_0|\mathcal{H}_1),
\end{align*}
meaning that the decoder wrongfully declares $\mathcal{H}_0$ --- the no error hypothesis.
 Therefore, with this setting the total probability of error for the transmission of a message is 
\begin{align}\label{eq: P_e in terms of P_eb}
P_e=\sum_{k=0}^{\infty} q^k P_{eb}=\frac{P_{eb}}{1-q}.
\end{align}
 
The number of blocks required to complete the transmission of one message is a geometric random variable with probability of success $1-q$. Thus, the expected number of blocks for transmission of a message is $\frac{1}{1-q}$. 
}
  %Observe that $P(\hat{\Theta}=\Theta_0)$ approaches $1$ as $n\rightarrow \infty$. Therefore,  the average transmission
%time approaches $1$ as $n\rightarrow \infty$. This implies that the average rate of transmission is $R_i=\frac{\log M_i}{n}, i=1,2$.
%Therefore, the expected number of channel uses for transmission of a message is $\EE[T]=\frac{n}{1-q}$. %As a result, the error exponent of the proposed scheme is 
%\begin{align*}
%\frac{-\log_2 P_e}{\EE[T]} =\frac{-\log_2 P_{eb}}{n(1-q)}+\frac{\log_2 (1-q)}{n(1-q)}. 
%\end{align*}

Next, we derive an upper-bound for $q$ and $P_{eb}$. 
%Error occurs if $\hat{\Theta}$ is not equal to the true hypothesis. It can be shown that the probability of error is dominated by $P(\Theta_1)P(\hat{\Theta}=\Theta_0 | \Theta_1 )$. The argument follows from a similar reasoning as in p.p.t channel.  
For shorthand,  denote $\Theta_{12}=(\Theta_1, \Theta_2), \hat{\Theta}_{12}=(\hat{\Theta}_1, \hat{\Theta}_2)$. Then
\begin{align*}
P_{eb}&=P\left(\hat{\Theta}_{12}=00, \Theta_{12}\neq 00\right)\\
&=\sum_{a\in \{01,10,11\}}P(\Theta_{12}=a)P(\hat{\Theta}_{12}=00|\Theta_{12}=a).
\end{align*}

Note that the effective rates of this transmission scheme are $(\frac{R_1}{1-\gamma}, \frac{R_2}{1-\gamma})$. If the effective rates are outside of the capacity region, then the probability of the error do not converge to zero. Hence, we need to choose $\gamma$, such that $(\frac{R_1}{1-\gamma}, \frac{R_2}{1-\gamma})$ is inside the feedback-capacity region of the channel.  From Corollary \ref{cor:fixed length capacity}, this happens if for any $\varepsilon \in (0,1)$, there exists $L\in \NN$ and $P^L\in \PMAC^L$ such that 
\begin{align*}
\frac{R_1}{(1-\gamma)} &\leq \frac{1}{L} I(X_1^L \rightarrow Y^L \|~ X^L_2)+\varepsilon\\
\frac{R_2}{(1-\gamma)} &\leq \frac{1}{L} I(X^L_2 \rightarrow Y^L \|~ X^L_1)+\varepsilon\\
\frac{R_1+R_2}{(1-\gamma)} &\leq \frac{1}{L}I(X^L_1, X^L_2 \rightarrow Y^L)+\varepsilon.
\end{align*}
For shorthand, let $I_L^1(P^L), I_L^2(P^L)$ and $I_L^3(P^L)$ denote, respectively, the normalized directed mutual information terms above. 
Then, $\gamma$ must be less than the following  
\begin{align}\label{eq: gamma^*}
\gamma^*= \sup_{L\in \NN, P^L\in \PMAC} \min_{i\in \set{1,2,3}} \set{1-\frac{R_i}{I_L^i(P^L)}},
\end{align}
where $R_3 =R_1+R_2$. As a result, with $\gamma \leq \gamma^*$,  there exist a sequence $\zeta_n , n\geq 1$ with $\zeta_n \rightarrow 0$ such that after the first stage $$\prob{\Theta_{12}\neq (0,0)} = P(\mathcal{H}_1) = \prob{(\hat{W}_1,\hat{W}_2)\neq (W_1,W_2)}\leq \zeta_n.$$ Hence, the probability of error is  bounded by
\begin{align} \label{eq: bound ofr P_e for confirmation stage}
P_{eb}&\leq  \sum_{a\in \{01,10,11\}} \zeta_n \prob{\hat{\Theta}_{12}=00|\Theta_{12}=a}.
\end{align}


\noindent\textbf{Analysis of the confirmation stage:}
Next, we analyze  $\prob{\hat{\Theta}_{12}=00|\Theta_{12}=a}$ as appearing in \eqref{eq: bound ofr P_e for confirmation stage}. First, consider $a=01$. Then, the condition for the decision region in \eqref{eq:log-like decision region} 
is equivalent to the following
\begin{align*}
\frac{1}{m}\log \frac{Q^m(y^m| \xHT{1}(0), \xHT{2}(0)) }{Q^m(y^m| \xHT{1}(0), \xHT{2}(1))} &= \frac{1}{m}\sum_{j=1}^m \log \frac{Q(y_j| x_{1,3,j}(0), x_{2,3, j}(0)) }{Q(y_j| x_{1,3, j}(0), x_{2,3,j}(1))}\\
& =  \sum_{u_1\in \mathcal{X}_1}\sum_{u_2,v_2\in \mathcal{X}_2} \mathsf{P}_m(u_1,u_2, *,v_2) \Big[ \sum_{s\in \mathcal{Y}} \hat{Q}_{\bfy}(s| u_1, u_2, v_2)   \log \frac{Q(s| u_1, u_2) }{Q(s| u_1, v_2)} \Big]\\
& =  \sum_{u_1\in \mathcal{X}_1}\sum_{u_2,v_2\in \mathcal{X}_2} \mathsf{P}_m(u_1,u_2, *,v_2) \Big[D\big( \hat{Q}_{\bfy}(\cdot | u_1, u_2, v_2)~\big\|~ Q(\cdot | u_1, v_2)\big)\\\numberthis \label{eq:decision reg1}
&\qquad  - D\big( \hat{Q}_{\bfy}(\cdot | u_1, u_2, v_2)~\big\|~ Q(\cdot | u_1, u_2)\big)\Big]
\end{align*}
Suppose $\underline{\bfZ}= (Z_1(0), Z_2(0), Z_1(1), Z_2(1))$ are random variables with joint distribution $\mathsf{P}_n$. 
Then, the right-hand side of \eqref{eq:decision reg1} equals to 
%\begin{align*}
% \EE_{P_m} \Big[D\big(\hat{Q}_{\bfy}(\cdot | X_1(0), X_1(1), X_2(0), X_2(1))~\big\|~ Q(\cdot | X_1(0), X_2(1))\big) - D\big(\hat{Q}_{\bfy}(\cdot | X_1(0), X_1(1), X_2(0), X_2(1))~\big\|~ Q(\cdot | X_1(0), X_2(0))\big)\Big]
%\end{align*}
\begin{align}\label{eq:decision KLD}
\frac{1}{m}\log \frac{Q^m(y^m| \xHT{1}(a_1), \xHT{2}(0)) }{Q^m(y^m| \xHT{1}(0), \xHT{2}(1))} = D\Big(\hat{Q}_{\bfy}(\cdot | \underline{\bfZ})\big\| Q(\cdot | Z_1(0), Z_2(1)) \big| \underline{\bfZ}\Big) - D\Big(\hat{Q}_{\bfy}(\cdot | \underline{\bfZ})\big\| Q(\cdot | Z_1(0), Z_2(0))\big| \underline{\bfZ}\Big)
\end{align}

We can derive similar expression for other values of $a=10,11$.
%\begin{align*}
%\KLdifbar\Big[\hat{Q}\| Q ~\big|~ a_1, a_2,  \mathsf{P}_m \Big]:= D\Big(\hat{Q}_{\bfy}(\cdot | \underline{\bfZ})~\big\|~ Q(\cdot | Z_1(0), Z_2(1)) \big| \underline{\bfZ}\Big) - D\big(\hat{Q}_{\bfy}(\cdot | \underline{\bfZ})~\big\|~ Q(\cdot | Z_1(0), Z_2(0))\big)\Big].
%\end{align*}
For any $a_1, a_2\in \set{0,1}$, define
\begin{align}\label{eq:Q lambda}
\mathcal{Q}_{\lambda}(a_1,a_2):= \set{\hat{Q}(y|\underline{\bfz})~:~  D\Big(\hat{Q}(\cdot | \underline{\bfZ})~\big\|~ Q(\cdot | Z_1(a_1), Z_2(a_2)) \big| \underline{\bfZ}\Big) - D\Big(\hat{Q}(\cdot | \underline{\bfZ})~\big\|~ Q(\cdot | Z_1(0), Z_2(0))\big| \underline{\bfZ}\Big) \geq \frac{\lambda}{m}},
\end{align}
For shorthand, we drop the subscript $\lambda$ in $\mathcal{Q}_{\lambda}(a_1,a_2)$. Therefore, the decision region corresponds to all sequences $y^m$ whose conditional type $\hat{Q}_{\bfy}$ belongs to $\medcap_{a\neq 00} \mathcal{Q}(a)$. Hence,  the error probability equals to 
\begin{align*}
\prob{\hat{\Theta}_{12}=00|\Theta_{12}=01} &= \prob{Y^m\in \mathcal{A}|\Theta_{12}=01}\\
&= \sum_{\hat{Q} \in \mathcal{Q}(a), \forall a\neq 00 }\sum_{\underline{x}\in T[\mathsf{P}_m]}\mathsf{P}_m(\underline{x})\sum_{y^m\in T_{\delta}^m(\hat{Q}(\cdot|\underline{x}))} Q^m(y^m| \underline{x_1}(0),\underline{x_2}(1))\\
&\leq   \sum_{\hat{Q} \in \mathcal{Q}(01)}\sum_{\underline{x}\in T[\mathsf{P}_m]}\mathsf{P}_m(\underline{x})\sum_{y^m\in T_{\delta}^m(\hat{Q}(\cdot|\underline{x}))} Q^m(y^m| \underline{x_1}(0),\underline{x_2}(1))\\
&= \sum_{\hat{Q} \in \mathcal{Q}(01) }\sum_{\underline{x}\in T[\mathsf{P}_m]}\mathsf{P}_m(\underline{x})\sum_{y^m\in T_{\delta}^m(\hat{Q}(\cdot|\underline{x}))}  \prod_{s, u_1, u_2, v_1, v_2} Q(s| u_1,v_2)^{m\mathsf{P}_m(u_1, v_1, u_2,v_2)\hat{Q}(s|u_1, v_1, u_2,v_2)}\\
&= \sum_{\hat{Q} \in \mathcal{Q}(01) }\sum_{\underline{x}\in T[\mathsf{P}_m]}\mathsf{P}_m(\underline{x})\sum_{y^m\in T_{\delta}^m(\hat{Q}(\cdot|\underline{x}))}  2^{ m\sum_{s, u_1, u_2, v_1, v_2} \mathsf{P}_m(u_1, u_2, v_1, v_2)\hat{Q}(s|u_1, u_2, v_1, v_2)    \log Q(s| u_1,v_2)}\\
&= \sum_{\hat{Q} \in \mathcal{Q}(01) }\sum_{\underline{x}\in T[\mathsf{P}_m]}\mathsf{P}_m(\underline{x})\sum_{y^m\in T_{\delta}^m(\hat{Q}(\cdot|\underline{x}))}  2^{ -m \EE_{P_m} \big[D(\hat{Q}(\cdot | \underline{\mathbf{X}})~\|~ Q(\cdot | X_1(0), X_2(1)))\big] -mH(\hat{Q}(\cdot | \underline{\bfX})) }\\
&\leq  \sup_{\hat{Q} \in \mathcal{Q}(01) } 2^{ -m \EE_{P_m} \big[D(\hat{Q}(\cdot | \underline{\bfX})~\|~ Q(\cdot | X_1(0), X_2(1)))\big]+\delta'}
\end{align*}
Using Chernoff-Stein's Lemma, we obtain that 
\begin{align*}
\prob{\hat{\Theta}_{12}=00|\Theta_{12}=01} \leq 2^{ -m \EE_{P_m} \big[D(Q(\cdot | X_1(0), X_2(0))~\|~ Q(\cdot | X_1(0), X_2(1)))\big]+\delta'}.
\end{align*}
For shorthand notation, define
\begin{align}\label{eq:dpar ij}
\bar{D}_{\mathsf{P}_m}(00||ij)=\EE_{\mathsf{P}_m}\Big[D_Q\big(X_1(0), X_2(0)|| X_1(i), X_2(j)\big)\Big], \quad \forall i,j \in \{0,1\} .
\end{align}
Then, using a similar argument, we have that 
%From the description of the transmission scheme, the codewords for the confirmation stage are selected with joint-type $\mathsf{P}_n$. In addition, the decoding process is performed using ML decoding. Therefore, the following bounds hold 
for $a\in \{01,10,11\}$:   
\begin{align*}
P(\hat{\Theta}_{12}=00|\Theta_{12}=a) \leq 2^{-n\gamma \bar{D}_{\mathsf{P}_m}(00||a)+\delta''}.
%P(\hat{H}_{12}=00|H_{12}=10) \leq 2^{-n\gamma D_Q(x_1(0), x_2(0)|| x_1(1), x_2(0))}\\
%P(\hat{H}_{12}=00|H_{12}=11) \leq 2^{-n\gamma D_Q(x_1(0), x_2(0)|| x_1(1), x_2(1))}
\end{align*}
Thus, from \eqref{eq: bound ofr P_e for confirmation stage}, the probability of error is upper bounded by 
\begin{align}\label{eq: bound on Pe}
P_{eb}&\leq 3  \zeta_n~ 2^{-n\gamma D_{lb,n}}
\end{align} 
Where $D_{lb,n}= \max_{\mathsf{P}_m}  \min_{a\in \{01,10,11\}} \bar{D}_{\mathsf{P}_m}(00||a)$. 

Next we derive an upper bound for $q$. We have 
\begin{align*}
q&=P(\hat{\mathcal{H}}=\mathcal{H}_1)\\
&=P(\mathcal{H}_0)P(\hat{\mathcal{H}}=\mathcal{H}_1|\mathcal{H}_0)+P(\mathcal{H}_1)P(\hat{\mathcal{H}}=\mathcal{H}_1|\mathcal{H}_1)\\
&\leq P(\hat{\mathcal{H}}=\mathcal{H}_1|\mathcal{H}_0)+\zeta_n,
\end{align*}
where the last inequality holds because of the following inequalities: (i) $P(\mathcal{H}_1)\leq \zeta_n$; (ii) $P(\mathcal{H}_0)\leq 1$; and  (iii) $P(\hat{\mathcal{H}}=\mathcal{H}_1|\mathcal{H}_1) \leq 1$. Note that 
\begin{align*}
 P(\hat{\mathcal{H}}=\mathcal{H}_1|\mathcal{H}_0)&=\sum_{a\in \{01,10,11\}} P(\hat{\Theta}_{12}=a|\Theta_{12}=00)\\
 &\leq \sum_{a\in \{01,10,11\}} 2^{-n\gamma \bar{D}_{\mathsf{P}_n}(a||00)}\\
 &\leq 3 \times 2^{-n\gamma \tilde{D}_{lb,n}},
\end{align*}
where $\tilde{D}_{lb,n}= \min_{a\in \{01,10,11\}} \bar{D}_{\mathsf{P}_n}(a||00)$. % It is assumed that $D_Q(x_1,x_2||z_1,z_2)>0$ for any $(x_1,x_2), (z_1,z_2) \in \mathcal{X}_1\times \mathcal{X}_2$ such that $(x_1,x_2)\neq (z_1,z_2)$. Under this condition, 
Therefore, there exists a sequence $\{q_n\}_{n\geq 1}$ with $q_n \rightarrow 0$ such that 
$q < q_n+\zeta_n$. Using this inequality and the inequality at \eqref{eq: bound on Pe}, we derive the following upper-bound for the total probability of error given in \eqref{eq: P_e in terms of P_eb} 
\begin{align*}
P_e \leq \frac{3 }{1-q_n-\zeta_n}  2^{-n\gamma D_{lb,n}}.
\end{align*}
%For any $\epsilon>0$, set $\gamma=\gamma^*-\epsilon$.
%In addition, 
 Therefore, the error exponent is bounded from below as 
\begin{align*}
\frac{-\log_2 P_e}{\EE[T]} &\geq \sup \frac{\gamma D_{lb,n}}{(1-q_n-\zeta_n)}+\xi_n
%&= \gamma^* D_{l},
\end{align*}
where $\xi_n=\frac{1}{n}\frac{\log_2(\frac{1-q_n-\zeta_n}{3})}{1-q_n-\zeta_n}$. Note that for any $\epsilon>0$ there exists large enough $n$ such that $q_n+\zeta_n<\epsilon, D_{lb,n}> D_{lb}-\epsilon, \xi_n <\epsilon$. Set $\gamma=\gamma^*-\epsilon$. Then
\begin{align*}
\frac{-\log_2 P_e}{\EE[T]} &\geq \gamma^* D_{lb}-\sigma(\epsilon)
\end{align*}
where $\sigma$ is a function of $\epsilon$ such that $\lim_{\epsilon \rightarrow 0}\sigma(\epsilon)=0$. Finally, the proof is complete by replacing $\gamma^*$ from \eqref{eq: gamma^*}.

%Note that $\mathsf{P}_n$ is an approximation of $P^*_{X_1X_2Z_1Z_2}$ that maximizes $D_l$. Lastly, the proof completes by the fact that $D_{l, n}$ approaches to $D_l$ as $n\rightarrow \infty$. 
\end{IEEEproof}


==> proofs/thm_proof_upperbound.tex <==
\section{Proof of Theorem \ref{thm: Error Exp Upper bound}}\label{appx: proof of thm Error Exp Upper bound}


\begin{proof}
Since $\{Z_t\}$ is a submartingale, then $Z_0 \leq \EE[Z_T]$. By the definition of $\{Z_t\}$  we have $\EE[Z_T]=\sum_{i=1}^3\alpha_i \EE[Z_T^i].$ For any of processes $\{Z^i_t\}$, the following hold:
\begin{align}\nonumber
\EE[Z^i_T]&=\EE \left[ \frac{H^i_T-\epsilon}{I^i_L+\epsilon}1_{\{H^i_T \geq \epsilon	\}}\right]+ \EE \left[ \left(\frac{\log H^i_T-\log \epsilon}{D_i+\epsilon}+f_i(\log \frac{H^i_T}{\epsilon})\right)1_{\{H^i_T \leq \epsilon\}}\right]+\EE[T]\\\nonumber
&\leq \EE \left[ \frac{H^i_T-\epsilon}{I^i_L+\epsilon}\right]+ \EE \left[\frac{\log H^i_T-\log \epsilon}{D_i+\epsilon}+f_i(\log \frac{H^i_T}{\epsilon})\right]+\EE[T]\\\nonumber
&\stackrel{(a)}{\leq} \EE \left[ \frac{H^i_T-\epsilon}{I^i_L+\epsilon}\right]+ \EE \left[\frac{\log H^i_T-\log \epsilon}{D_i+\epsilon}\right]+\frac{1}{\mu_i D_i}+\EE[T]\\\nonumber
& = \frac{\EE[H^i_T]-\epsilon}{I^i_L+\epsilon}+ \frac{\EE[\log H^i_T]-\log \epsilon}{D_i+\epsilon}+\frac{1}{\mu_i D_i}+\EE[T]\\\label{eq: bound on E[Z_T^i]}
&\stackrel{(b)}{\leq}  \frac{\EE[H^i_T]-\epsilon}{I^i_L+\epsilon}+ \frac{\log \EE[H^i_T]-\log \epsilon}{D_i+\epsilon}+\frac{1}{\mu_i D_i}+\EE[T]
\end{align}
where $(a)$ follows from the inequality $f_i(y)\leq \frac{1}{\mu_i D_i} $, and $(b)$ follows by applying Jensen's inequality for the function $\log(x)$.

Define $\eta(P_e)=h_b(P_e) + P_e \log(M_1M_2)$. Using Lemma \ref{lem: generalized fano for MAC-FB}, the right-hand side of \eqref{eq: bound on E[Z_T^i]} is upper bounded as 
\begin{align}\nonumber
&\leq \frac{\eta(P_e)-\epsilon}{(I^i_L+\epsilon)}+ \frac{\log (\eta(P_e))-\log \epsilon}{D_i+\epsilon}+\frac{1}{\mu_i D_i}+\EE[T]\\\nonumber
&= \frac{\eta(P_e)-\epsilon}{(I^i_L+\epsilon)}+ \frac{\log P_e + \log \frac{\eta(P_e)}{P_e}-\log \epsilon}{D_i+\epsilon}+\frac{1}{\mu_i D_i}+\EE[T]\\\label{eq: bound 2 on E[Z_T]}
&\leq \frac{\log P_e}{D_i+\epsilon} +\EE[T](1 + \delta_i(P_e, M_1M_2, \epsilon)),
\end{align}
where the function $\delta_i$ is defined as 
\begin{align*}
\delta_i(& P_e, M_1M_2, \epsilon)= \|  \frac{\eta(P_e)-\epsilon}{(I^i_L+\epsilon) \frac{\log M_1M_2}{R^{(3)}_N}}+ \frac{\log \frac{\eta(P_e)}{P_e}-\log \epsilon}{(D_i+\epsilon) \frac{\log M_1M_2}{R^{(3)}_N}}+\frac{1}{\mu_i D_i\frac{\log M_1M_2}{R^{(3)}_N}}\|
\end{align*}
Note that we use the equation $\EE[T]=\frac{\log M_1M_2}{R^{(3)}_N}$ in the definition of $\delta_i$. Observe that   $$\lim_{P_e\rightarrow 0 } \lim_{M_1M_2 \rightarrow \infty} \delta_i(P_e, M_1M_2, \epsilon)=0.$$ %Thus, from \eqref{eq: bound 2 on E[Z_T]} and the definition of $\{Z_t\}$ we obtain
%\begin{align}\nonumber
%\EE[Z_T] &\leq \sum_{i=1}^3 \log P_e \frac{ \alpha_i}{D_i+\epsilon} +\alpha_i \EE[T] ( 1 + \delta_i(P_e, M_1M_2, \epsilon))\\\label{eq: last bound on E[Z_T]}
%&\leq   \frac{ \log P_e }{D_{min}} +\EE[T] ( 1 + \sum_{i=1}^3\delta_i(P_e, M_1M_2, \epsilon)),
%\end{align}
%where  $D_u\triangleq \min\{\bar{D}^1_{\mathsf{P}},\bar{D}^2_{\mathsf{P}},\bar{D}^3_{\mathsf{P}}\}$. 
Note that $Z_0^i \leq \EE[Z_T^i], i=1,2,3$, where
$Z_0^i =  \frac{\log M_i-\epsilon}{I_L^i+\epsilon}.$
Therefore, 
\begin{align*}
\frac{\log M_i-\epsilon}{I_L^i+\epsilon} \leq \frac{\log P_e}{D_i+\epsilon}+\EE[T] ( 1 +  \delta_i(P_e, M_1M_2, \epsilon))
\end{align*}
Multiplying both sides by $\frac{D_i+\epsilon}{\EE[T]}$ and rearranging the terms give 

\begin{align*}
-\frac{\log P_e}{\EE[T]}& \leq  (D_i+\epsilon)\left(1-\frac{R^{(i)}_N}{I_L^i+\epsilon}\right)\\
&+\frac{\epsilon (D_i+\epsilon)}{(I_L^i+\epsilon)\EE[T]}+{(D_i+\epsilon)} \delta_i(P_e, M_1M_2, \epsilon),
\end{align*}

\red{[AA: At this point we have a pretty intuitive bound as follows (I am omitting small terms)
\begin{align*}
-\frac{\log P_e}{\EE[T]}& \leq  \min_i D_i\left(1-\frac{R^{(i)}_N}{I^i_L}\right).
\end{align*}
The next intuitive step is to maximize over all input multi-dimensional distributions (codes) to get the final bound
\begin{align*}
E& \leq  \sup_{P}\min_i D_i\left(1-\frac{R^{(i)}_N}{I^i_L}\right).
\end{align*}
This is very intuitive, but it has one problem: it has decomposed the dependence of $D_i$ from $P$ ($P$ affects only $I^i_L$).
We can fix this: we can go back to Lemma~8 and use a softer bound of the form $D_1(P)< D_1$. This essentially says that when user~2 transmits information (eg, relevant to phase~2 in a 3-phase system) user~1 cannot get the smallest decay $D_1$ but only $D_1(P)$ so there is a tradeoff between $D_i(P)$ and $I^i(P)$.
]}

Define
\begin{align*}
\tilde{\delta}(P_e, M_1M_2, \epsilon)=\max_i \frac{(D_i+\epsilon) ~ \epsilon ~R^{(3)}_N}{(I_L^i+\epsilon') \log M_1M_2}+(D_i+\epsilon) \delta_i(P_e, M_1M_2, \epsilon).
\end{align*}

For any non-negative numbers $\lambda_i, i=1,2,3$ the following inequality holds:
\begin{align*}\numberthis \label{eq: bound on Exp as D_i}
-\frac{\log P_e}{\EE[T]}&  \leq  (D_i+\epsilon)\left(1- \frac{R^{(i)}_N}{I_L^i+\epsilon}\right)+\tilde{\delta},\\
&\leq  (D_i+\epsilon)\left(1-\frac{\lambda_i R^{(i)}_N}{\lambda_i I_L^i+\epsilon}\right)+\tilde{\delta},\\
&\leq  (D_i+\epsilon)\left(1-\frac{\lambda_i R^{(i)}_N}{\sum_j \lambda_j I_L^j+\epsilon'}\right)+\tilde{\delta},\\
&\leq  (D_i+\epsilon) \left(1-\frac{\lambda_i R^{(i)}_N}{\sup \sum_j \lambda_j I_L^j+\epsilon}\right)+\tilde{\delta},\\
&=  (D_i+\epsilon)\left(1-\frac{\lambda_i R^{(i)}_N}{C_{\lambda}+\epsilon}\right)+\tilde{\delta},
\end{align*}
Since the transmission rates are inside the capacity region, $\lambda_i R^{(i)}_N \leq C_{\lambda}$ and we obtain 
\begin{align*}
\frac{\log P_e}{\EE[T]}&  \leq  D_i\left(1-\frac{\lambda_i R^{(i)}_N}{C_{\lambda}+\epsilon}\right)+\epsilon+\tilde{\delta}(P_e, M_1M_2, \epsilon),\\
& \stackrel{(a)}{=}  D_i\left(1-\frac{\lambda_i R^{(i)}_N}{C_{\lambda}}\right)+ D_i \frac{\lambda_i R^{(i)}_N\epsilon}{C_{\lambda}(C_{\lambda}+\epsilon)} + \epsilon+\tilde{\delta}(P_e, M_1M_2, \epsilon),\\
& \stackrel{(b)}{\leq}  D_i\left(1-\frac{\lambda_i R^{(i)}_N}{C_{\lambda}}\right)+ D_{\max} \frac{\epsilon}{C_{\lambda}} + \epsilon+\tilde{\delta}(P_e, M_1M_2, \epsilon),\\
\end{align*}
where $D_{\max}=\max\{D_1, D_2, D_3\}$, (a) follows by adding and subtracting the term $D_i(\frac{\lambda_i R^{(i)}_N}{C_{\lambda}})$, and (b) follows as $\frac{\lambda_i R^{(i)}_N}{C_{\lambda}+\epsilon}\leq 1$. Define ${\delta}(P_e, M_1M_2, \epsilon)= \epsilon(1+  \frac{D_{\max}}{C_{\lambda}})+\tilde{\delta}(P_e, M_1M_2, \epsilon)$. The theorem follows by taking the minimum over $\lambda_i, i=1,2,3$ and the fact that the following condition is satisfied: $$\lim_{\epsilon \rightarrow 0}\lim_{P_e \rightarrow 0}\lim_{M_1M_2 \rightarrow \infty} \delta(P_e, M_1M_2, \epsilon)=0.$$ 
Note that in the above proof it is assumed that the capacity region is nonempty. This assumption implies that $C_{\lambda}>0$ for all $\underline{\lambda}\neq \underline{0}$ with non-negative components.   
\end{proof}

\section{Proof of Corollary \ref{cor: Exp upper bound}}\label{app: proof corrolary Exp upper bound}
From \eqref{eq: bound on Exp as D_i} in the proof of Theorem \ref{thm: Error Exp Upper bound}, we obtain: 
\begin{align*}
-\frac{\log P_e}{\EE[T]}&  \leq \min_{i \in \{1,2,3\}} (D_i+\epsilon)\left(1- \frac{R^{(i)}_N}{I_L^i+\epsilon}\right)+\tilde{\delta}\\
&\leq D_{\max}\min_{i \in \{1,2,3\}} \left(1- \frac{R^{(i)}_N}{I_L^i}\right)+\delta\\\numberthis \label{eq: cor bound i}
&= D_{\max} \min_{\substack{\alpha_1, \alpha_2, \alpha_3 \geq 0\\ \alpha_1+\alpha_2+\alpha_3=1}} \left(1- \sum_{i=1}^3 \alpha_i\frac{R^{(i)}_N}{I_L^i}\right)+{\delta},
\end{align*}
where $D_{\max}=\max\{D_1,D_2,D_3\}$, and $\delta=\tilde{\delta}+\epsilon \sup (1+\frac{D_{\max}}{I_L^i})$. For non-negative $\lambda_i, i=1,2,3$, set 
$\alpha_i = \frac{\lambda_i I_L^i}{\sum_j \lambda_j I_L^j}.$
Next, replace $\alpha_i, i=1,2,3$ in \eqref{eq: cor bound i} with the above term. Therefore, \eqref{eq: cor bound i} does not exceed the following
\begin{align*}
 &D_{\max} \min_{\substack{\lambda_1, \lambda_2, \lambda_3 \geq 0\\ \lambda_1+\lambda_2+\lambda_3=1}} \left(1-  \frac{\sum_{i}\lambda_i R^{(i)}_N}{\sum_j \lambda_j I_L^j}\right)+{\delta}.
\end{align*}
The proof is completed by noting that $\sum_j \lambda_j I_L^j \leq C_{\lambda} $.  

==> references.tex <==
\begin{thebibliography}{1}
\bibitem{Shannon_zero}
C. E. Shannon. The zero error capacity of a noisy channel. IRE Trans. on Inform. Th., 2(3):8–19, 1956

\bibitem{Burnashev}
M. V. Burnashev, ``Data transmission over a discrete channel with feedback. Random transmission time,” Problemy Peredachi Informatsii, vol. 12, no. 4, pp. 10–30, Oct.-Dec. 1976.


\bibitem{Schalkwijk-Kailath}
 J. Schalkwijk and T. Kailath, “A coding scheme for additive noise channels with feedback–I: No bandwidth constraint,” IEEE Trans. Info. Theory, vol. 12, no. 2, pp. 172–182, Apr 1966.

\bibitem{Dobrushin}
 R. L. Dobrushin, “An asymptotic bound for the probability error of information transmission through a channel without memory 	using the feedback,” Problemy Peredachi Informatsii, vol. 8, pp. 161–160, 1962.

\bibitem{Haroutunian}
E. A. Haroutunian, “Lower bound for error probability in channels with feedback,” Problemy Peredachi Informatsii, vol. 13, pp. 36–44, 1977.

\bibitem{Berlin}
P. Berlin, B. Nakiboglu, B. Rimoldi, and E. Telatar, “A simple converse of burnashev’s reliability function,” IEEE Trans. Info. Theory, vol. 55, no. 7, pp. 3074–3080, July 2009.

\bibitem{Yamamoto}
H. Yamamoto and K. Itoh, ``Asymptotic performance of a modified schalkwijk-barron scheme for channels with noiseless feedback (corresp.),” IEEE Trans. Info. Theory, vol. 25, no. 6, pp. 729–733, Nov 1979.


\bibitem{Gaarder-Wolf}
N. T. Gaarder and J. K. Wolf, ``The capacity region of a multiple-access discrete memoryless channel can increase with feedback," IEEE Trans. Inf. Theory, vol. 21, no. 1, pp. 100–102, 1975.

\bibitem{Willems-FB}
F. M. J. Willems, ``The feedback capacity region of a class of discrete memoryless multiple access channels," IEEE Trans. Inf. Theory, vol. 28, no. 1, pp. 93–95, 1982.


\bibitem{Kramer-thesis}
G. Kramer, Directed Information for channels with Feedback. PhD
thesis, Swiss Federal Institute of Technology, Zurich, 1998.



%\bibitem{Ozarow}
%L. H. Ozarow, ``The capacity of the white Gaussian multiple access
%channel with feedback," IEEE Trans. Inf. Theory, vol. 30, no. 4, pp. 623–628, 1984.

\bibitem{EX-BC}
L. V. Truong and V. Y. F. Tan, ``Error exponent of the common-message broadcast channel with variable-length feedback," IEEE Int. Symp. on Info. Theory (ISIT), Aachen, 2017, pp. 186-190.


%\bibitem{Lapidoth}
%S. Bross and A. Lapidoth, ``An improved achievable region for the discrete memoryless two-user multiple-access channel with noiseless
%feedback," IEEE Trans. Inf. Theory, vol. IT-51, pp. 811–833, March 2005.

%\bibitem{Ramji-Sandeep-FB}
%R. Venkataramanan and S. S. Pradhan, ``A New Achievable Rate Region for the Multiple-Access Channel With Noiseless Feedback," in IEEE Trans. on Info. Theory, vol. 57, no. 12,  pp. 8038-8054, Dec. 2011.


%\bibitem{Kramer-DMN}
%G. Kramer, ``Capacity Results for the Discrete Memoryless Network,"
%IEEE Trans. Inf. Theory, vol. 49, pp. 4–20, January 2003.
\bibitem{ISIT17-FB}
M. Heidari, F. Shirani and S. S. Pradhan, ``On the necessity of structured codes for communications over MAC with feedback," IEEE Int. Symp. on Info. Theory (ISIT), Aachen, 2017, pp. 2298-2302.

\bibitem{nazari-MAC-FB-UB}
A. Nazari, S. S. Pradhan and A. Anastasopoulos, ``Error Exponent for Multiple Access Channels: Upper Bounds," in IEEE Trans. Info. Theory, vol. 61, no. 7, pp. 3605-3621, July 2015.

%\bibitem{nazari-MAC-FB-LB}
%A. Nazari, A. Anastasopoulos and S. S. Pradhan, "Error Exponent for Multiple-Access Channels: Lower Bounds," in IEEE Transactions on Information Theory, vol. 60, no. 9, pp. 5095-5115, Sept. 2014.

\bibitem{Gallager}
 R. Gallager, ``A perspective on multi-access channels," IEEE Trans. Information Theory, vol. 31, pp. 124–142, Mar. 1985.
%\bibitem{Arxiv-version}
%M. Heidari, A. Anastasopoulos and S. S. Pradhan, ``On The Reliability Function of Discrete Memoryless Multiple-Access Channel with Feedback," https://arxiv.org/, 2018. 
%%\bibitem{Massey}  J. L. Massey, “Causality, feedback and directed information,” in Proc.
%%1990 IEEE Int. Symp. Information Theory and Its Applications, Hawaii,
%%Nov. 27–30, 1990, pp. 303–305.
%%

\end{thebibliography}

==> upper_bound_twophase.tex <==
\subsection{Two-phase Upper-bound}\label{sec:up two phase}


%\subsection{Converse for the Reliability Function}
In this part of the paper, we establish an upper-bound for the reliability function of any discrete memoryless MAC.
Define
\begin{align}\label{eq: definiton of D_i}
D_i&\triangleq \max_{\substack{x_1, z_1\in \mathcal{X}_1,\\ x_2,z_2 \in \mathcal{X}_2}} D_i(x_1,x_2||z_1, z_2), \quad i=1,2,3.
\end{align}

%\begin{theorem}[Upper-bound]\label{thm: Error Exp upper-bound}
%For any $(N, M_1,M_2)$ VLC with probability of error $P_e$, there exist $\delta>0$ (as a function of $P_e, M_1,M_2$)  such that the following is an upper-bound for the reliability function of this VLC
%\begin{align}\label{eq: E_u}
%E_u(R_1,R_2)= \min_{\substack{\lambda_1, \lambda_2, \lambda_3 \geq 0\\ \lambda_1+\lambda_2+\lambda_3=1}} \left( 1-\frac{\sum_{i=1}^3\lambda_iR_i}{C_{\lambda}}  \right) D_u+ \delta 
%\end{align}
%where $D_u=\min\{D_1,D_2\}$, and $\delta$ is a function such that $$\lim_{P_e\rightarrow 0}\lim_{M_1M_2\rightarrow \infty} \delta(P_e,M_1M_2)=0$$
%\end{theorem}
\begin{theorem}[Upper-bound]\label{thm: Error Exp Upper bound}
For any $(N, M_1,M_2)$ VLC with probability of error $P_e$, and any $\epsilon>0$, there exists a function $\delta$ such that the following is an upper-bound for the reliability function of the VLC
\begin{align}\nonumber
E(R_1,R_2)\leq &\min_{\substack{\lambda_1, \lambda_2, \lambda_3 \geq 0\\ \lambda_1+\lambda_2+\lambda_3=1}}\min_{j\in \{1,2,3\}} D_j \left(1- \frac{\lambda_j R_j}{C_{\lambda}}\right)\\\label{eq: E_u} &+\delta(P_e, M_1M_2, \epsilon),
\end{align}
where $(R_1, R_2)$ is the rate pair of the VLC and $\delta$ satisfies $$\lim_{\epsilon\rightarrow 0} \lim_{P_e\rightarrow 0}\lim_{M_1M_2\rightarrow \infty} \delta(P_e,M_1M_2, \epsilon)=0.$$
\end{theorem}

\begin{corollary}\label{cor: Exp upper bound}
From Theorem \ref{thm: Error Exp Upper bound}, the following is an upper-bound for the error exponent of a MAC: 
\begin{align}\nonumber
E_u(R_1,R_2)=& \min_{\substack{\lambda_1, \lambda_2, \lambda_3 \geq 0\\ \lambda_1+\lambda_2+\lambda_3=1}}D_{u} \left(1-\frac{\sum_{i=1}^3  \lambda_i R_i}{C_{\lambda}}\right)+\delta,
\end{align}
where $D_u=\max\{D_1, D_2, D_3\}$, and $\delta$ is as in Theorem \ref{thm: Error Exp Upper bound}.
\end{corollary}
\begin{IEEEproof}
The proof is given in Appendix \ref{app: proof corrolary Exp upper bound}. 
\end{IEEEproof}
%The proof of the theorem is presented in Subsection \ref{subsec: proof of theorem}. 

%\input{Proof_thm_upperbound_Berline.tex}

%\input{Proof_thm_upperbound_Burnashev}

